CTAB-GAN+: Enhancing Tabular Data Synthesis

While data sharing is crucial for knowledge development, privacy concerns and strict regulation (e.g., European General Data Protection Regulation (GDPR)) limit its full effectiveness. Synthetic tabular data emerges as alternative to enable data sharing while fulfilling regulatory and privacy constraints. State-of-the-art tabular data synthesizers draw methodologies from Generative Adversarial Networks (GAN). As GANs improve the synthesized data increasingly resemble the real data risking to leak privacy. Differential privacy (DP) provides theoretical guarantees on privacy loss but degrades data utility. Striking the best trade-off remains yet a challenging research question. We propose CTAB-GAN+ a novel conditional tabular GAN. CTAB-GAN+ improves upon state-of-the-art by (i) adding downstream losses to conditional GANs for higher utility synthetic data in both classification and regression domains; (ii) using Wasserstein loss with gradient penalty for better training convergence; (iii) introducing novel encoders targeting mixed continuous-categorical variables and variables with unbalanced or skewed data; and (iv) training with DP stochastic gradient descent to impose strict privacy guarantees. We extensively evaluate CTAB-GAN+ on data similarity and analysis utility against state-of-the-art tabular GANs. The results show that CTAB-GAN+ synthesizes privacy-preserving data with at least 48.16% higher utility across multiple datasets and learning tasks under different privacy budgets.

==> background.tex <==
\section{Related Studies}
We divide the related studies using GAN to generate tabular data into two categories: (i) based on GAN, and (ii) based on conditional GAN.
%Synthetic data study has attracted both interests from academia and industry. It becomes especially important as more regulations implemented on data sharing and data usage. The difficulties of generating realistic tabular data are, in one hand, the synthetic data should has as close as possible statistic distributions as original data, and similar utility when being used to build models. In another hand, we need to prevent attackers to infer original data from synthetic data.

%\lc{shorten it}%Since GAN~\cite{gan} is proposed, %GAN and their numerous extensions [], 
% it has gained great attentions due to the performance and flexibility offered in representing data. Although GAN shows promising results in many applications, it is known for its difficulty in training. Many GAN models suffer the problems such as: (1) non-convergence, (2) mode collapse and (3) diminished gradient. To address these problems, Wasserstein GAN~\cite{wgan} is first proposed. Later on, its successive works such as Cramér distance based GAN~\cite{cramerdistance} and Wasserstein GAN plus gradient penalty~\cite{wgan_gp} all improve the training stability of GAN. 
%\cite{wgan} proposes using Wasserstein distance instead of the Jensen-Shannon divergence (JSD) to measure the distance between the model distribution and the real distribution. \cite{wgan} also illustrates that if the generated data distribution is far away from the ground truth distribution of real data, the generator barely learns anything based on JSD. \cite{cramerdistance} points out that, when using stochastic gradient descent (SGD) based optimizer, estimating the Wasserstein metric from samples yields biased gradients, and may actually lead to the wrong minimum. Therefore, they propose the Cramér distance which not only keeps the good properties of Wasserstein distance, but also overcomes the problem of biased sample gradients. \cite{wgan_gp} also addresses the problem in~\cite{wgan} which occasionally produces poor sample or fail to converge. They find that these problems are often due to the use of weight clipping in Wasserstein GAN (WGAN) to enforce a Lipschitz constraint on the critic, which can lead to undesired behavior. They propose an alternative to clipping weights: penalize the norm of gradient of the critic with respect to its input.
 

%Most of GAN-based applications are focused on generating high resolution images, but some are also used in generating tabular data. 
%Above researches are focusing on improving the stability of GAN structure, back to our tabular data synthesis, we still have the domain-related difficulties. 
\textbf{GAN-based generator}. Several studies extend GAN to accommodate categorical variables by augmenting GAN architecture. 
MedGAN (\cite{medgan}) combines an auto-encoder with a GAN. It can generate continuous or discrete variables, and has been applied to generate synthetic electronic health record (EHR) data. CrGAN-Cnet (\cite{cramergan}) uses GAN to conduct Airline Passenger Name Record Generation. It integrates the Cramér Distance (\cite{cramerdistance}) and Cross-Net architecture (\cite{crossnet}) into the algorithm. In addition to generating with continuous and categorical data types,  CrGAN-Cnet can also handle missing value in the table by adding new \columns. TableGAN (\cite{tablegan}) introduces information loss and a classifier into GAN framework. It specifically adopts Convolutional Neural Network (CNN) for generator, discriminator and classifier. 
%uses Convolutional Neural Network (CNN) as generator to generate synthetic tabular data. They also add an additional neural network classifier to increase the \textbf{semantic integrity} of synthetic records. For instance, (sex=man, disease=uterine cancer) is not a semantically correct record as man does not have uterine, and there should not contain such record in the original table. A classifier can help to prevent the generation of such records. 
Although aforementioned algorithms can generate tabular data, they cannot specify how to generate from a specific class for particular variable. For example, it is not possible to generate health record for users whose sex is female. %  to generate the data (e.g., only generate EHR for whose sex is female.).
In addition to data generation, privacy is another important factor for synthetic tabular data. PATE-GAN (\cite{pategan}) is not specifically designed for tabular data generation, but it proposes a framework which generates  synthetic  data  with  differential  privacy  guarantees.
%\lc{Add a flow to connect this reference}


\textbf{Conditional GAN-based generator}. Due to the limitation of controlling generated data via GAN, Conditional GAN is increasingly used, and its conditional vector can be used to specify to generate a particular class of data. This feature is important when our available data is limited and highly skewed, and we need synthetic data of a specific class to re-balance the distribution. For instance, for preparing starting dataset of online learning scenarios (\cite{Zhao:DSN19,Zhao:TDSC21,younesian2020qactor}). CW-GAN (\cite{cwgan}) applies the Wasserstein distance (\cite{wgan}) into the conditional GAN framework. It leverages the usage of conditional vector to oversample the minority class to address imbalanced tabular data generation. CTGAN (\cite{ctgan}) integrates PacGAN (\cite{pacgan}) structure in its discriminator and uses Generator loss and WGAN loss plus gradient penalty (\cite{wgan_gp}) to train a conditional GAN framework. It also adopts a strategy called training-by-sampling, which takes advantage of conditional vector, to deal with the imbalanced categorical variable problem. 
%\lc{Stress the coding and the difference with what we have done compared to the related work}
In our paper, we not only focus on modelling continuous or categorical variables, but also cover the \mixed data type (i.e., \columns that contain both categorical and continuous values, or even missing values). We effectively combine the strengths of prior art, such as classifier, information, generator loss, effective encoding, and conditional vector. Furthermore, we proactively address the pain point of long tail \variable distributions %. predominant  Generation problem of long-tailed
and propose a new conditional vector structure to better deal with imbalanced datasets.
\color{blue}

\textbf{Differential Private Tabular GANs}.
To avoid leaking sensitive information on single individuals, related work explored several possibilities to provide differential privacy guarantees with GANs. Table~\ref{table:DD} provides an overview across the main ingredients used. Both of the two private learning techniques have been applied. PATE-GAN~\cite{pategan} uses PATE~\cite{papernot2016semi} which relies on output sanitization perturbing the output of an ensemble of teacher discriminators via Laplacian noise to train a student discriminator scoring the generated samples from the generator. One key limitation is that the student discriminator only sees synthetic data. Since this data is potentially unrealistic the provided feedback can be unreliable. \cite{xie2018differentially} (DP-WGAN), \cite{chen2020gs} (GS-WGAN) and \cite{torfi2020differentially} (RDP-GAN) use DP-SGD coupled with the Wasserstein loss. Moreover, \cite{xie2018differentially} uses a momentum accountant whereas \cite{chen2020gs,torfi2020differentially} a R\'enyi differential privacy accountant. 

The Wassertein loss is known to be more effective against mode-collapse as compared to KL divergence~\cite{pmlr-v70-arjovsky17a}. The RDP accountant provides tighter bounds on the privacy costs improving the privacy-utility tradeoff.
To incorporate differential privacy guarantees and make the training compatible with the Wasserstaien Loss~\cite{xie2018differentially,torfi2020differentially} use weight clipping to enforce the Lipschitz constraint. The drawback is the need for careful tuning of the clipping parameter, see Sec.~\ref{ssec:dp-sgd}. To overcome this issue, \cite{chen2020gs} enforces the Lipschitz constraint via a gradient penalty term as suggested by~\cite{gulrajani2017improved}, but addresses only images which are a better fit for GANs and studies its efficacy only for training the generator network. 

The proposed \system leverages RDP-based privacy accounting as well as the Wasserstein loss with a gradient penalty for improved privacy accounting and training stability, respectively. However, different from related work, we tackle differential privacy at both generator, \systemg, and discriminator, \systemd, to investigate the most optimal site for integrating DP in tabular GANs. Moreover, we elucidate the privacy cost associated with complex loss functions (i.e., classification and information losses) used by the generator for enhancing the quality of synthetic tabular datasets. Additionally we experimentally show that spherical interpolates are a better alternative than linear interpolates for computing the gradient penalty associated with the Wasserstein loss to further improve training performance under strict privacy budgets.
\color{black}
\begin{table}[t]
\caption{Overview of related work.}
\resizebox{\columnwidth}{!}{
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Model}} & \textbf{DP Algo} & \textbf{Loss$^*$} &\textbf{DP Site} & \textbf{Noise}& \textbf{Account.} & \textbf{Data Format}\\ 
\hline
\multicolumn{2}{|c|}{PATE-GAN} & PATE & KL Diver.  &  $\mathcal{D}$   & $\text{Lap}()$  & PATE & Table\\\hline
\multicolumn{2}{|c|}{DP-WGAN} & DP-SGD & Was. + WC    &  $\mathcal{D}$   & $\mathcal{N}$  & Moment & Image $\&$ Table \\ \hline
\multicolumn{2}{|c|}{GS-WGAN} & DP-SGD & Was. + GP & $\mathcal{G}$  & $\mathcal{N}$ & RDP & Image\\ \hline

\multicolumn{2}{|c|}{RDP-GAN} & DP-SGD & Was. + WC & $\mathcal{D}$  & $\mathcal{N}$ & RDP & Table\\ \hline

\multirow{2}{*}[-0.1em]{\begin{sideways}\bf Ours\end{sideways}} 
& \systemd & DP-SGD & Was. + GP   &  $\mathcal{D}$  & $\mathcal{N}$  & RDP  & Table\\
\cline{2-8} 
& \systemg & DP-SGD & Was. + GP    &  $\mathcal{G}$   & $\mathcal{N}$  & RDP  & Table \\ \hline
\multicolumn{8}{l}{$^*$ Was. (Wasserstein), WC (Weight Clipping), GP (Gradient Penalty)} \\
\end{tabular}
}
\label{table:DD}
\end{table}

% \iffalse
% \begin{table*}[ht]
%   \centering
%     \begin{tabular}{l|SS|c|c|c|SSS}
%          \rowcolor{gray!25}                                                     & \multicolumn{2}{c|}{\bf Architecture}   &                                     &                               &                            & \multicolumn{3}{c}{\bf Resource aware} \\
%          \rowcolor{gray!25} \multirow{-2}{*}{\bf Method}                        & {GPU}       & {CPU}                     & \multirow{-2}{*}{\bf Multi-DNNs}   & \multirow{-2}{*}{\bf Response Time} & \multirow{-2}{*}{\bf Edge} &  {Memory} & {Energy} & {Temperature} \\ \hline
%          MCDNN \cite{Han2016MCDNN:Constraints}                                  & \cmark      & \cmark                    &  \cmark                            &                                & \cmark~/ \xmark            & \cmark   & \cmark   & \xmark        \\
%          DeepEye \cite{Mathurz2017DeepEye:Hardware}    & \xmark      & \cmark                    &  \cmark                            &                                & \cmark                     &          &          &               \\
%          NeuOS \cite{bateni2020neuos}                                           &             &                           &                                    &                                &                            &          &          &               \\
%          NestDNN \cite{Fang2018NestDNN:Vision}                                  &             &                           &  \cmark                            &                                & \cmark                     & \cmark   & \xmark   & \xmark        \\
%          DeepMon \cite{huynh2017deepmon}                                        &             &                           &                                    &                                &                            &          &          &               \\
%          {\bf EdgeCaffe}                                                        & \xmark      & \cmark                    &  \cmark                            & \cmark                         & \cmark                     & \cmark   & \cmark   & \cmark        \\ \hline
%     \end{tabular}
%     % \rowcolors{2}{gray!10}{white}
%     \caption{Overview of prior-art}
%     \label{tab:comparison_table}
% \end{table*}

==> experiment.tex <==
\section{Experimental Analysis for Data utility}

To show the efficacy of the proposed \algoplus, we select five commonly used machine learning datasets, and compare with four state-of-the-art GAN based tabular data generators. We evaluate the effectiveness of \algoplus in terms of the resulting ML utility, statistical similarity to the real data, and privacy distance.  Moreover, we provide an ablation analysis to highlight the efficacy of the unique components of \algo.

\subsection{Experimental Setup}
\label{ssec:setup}
% \subsubsection{Datasets:} 

%\quad \; 
{\bf Datasets}. Our algorithm is tested on five commonly used machine learning datasets. Three of them    \textbf{Adult}%\footnote{http://archive.ics.uci.edu/ml/datasets/adult}
, \textbf{Covertype}
 %\footnote{https://archive.ics.uci.edu/ml/datasets/covertype}
 and \textbf{Intrusion} %\footnote{http://archive.ics.uci.edu/ml/datasets/kdd+cup+1999+data}
 are from the UCI machine learning repository\footnote{\url{http://archive.ics.uci.edu/ml/datasets}}.
 %(\cite{UCIdataset}). 
 The other two \textbf{Credit} %\footnote{\url{https://www.kaggle.com/mlg-ulb/creditcardfraud}} 
 and \textbf{Loan} %\footnote{\url{https://www.kaggle.com/itsmesunil/bank-loan-modelling}}  
 are from Kaggle\footnote{\url{https://www.kaggle.com/{mlg-ulb/creditcardfraud,itsmesunil/bank-loan-modelling}}}. All five tabular datasets have a target \column, for which we use the rest of the \columns to perform classification. Due to computing resource limitations, 50K rows of data are sampled randomly in a stratified manner with respect to the target \column for Covertype, Credit and Intrusion datasets.  %\lc{Be more precise on "maintaing the original distribution"} 
 However, the Adult and Loan datasets are not sampled. The details of each dataset are shown in Tab.~\ref{table:DD}. One thing to notice is that we assume that the user already knows the data type of each variable before training. \cite{ctgan} holds the same assumptions.
%Note that the Adult, Credit and Loan datasets belong to the binary classification problem domain whereas the covertype dataset along with the Intrusion dataset reside in the multi-class classification problem setting
% \lc{All cpations should be on the top of all figures}
\begin{table*}[t]
\centering
%\caption{Description of datasets. The notations $C$, $B$, $M$ \& $Mi$ represent number of continuous, binary, multi-class categorical, and \mixed \variables.}
\caption{Description of Datasets.}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{ |c|c|c|c|c|c|c|c|c| }
\hline
\textbf{Dataset} & \textbf{Problem}& \textbf{Train/Test Split} &\textbf{Target \column} & \textbf{$\mbox{Continuous}$}  & \textbf{$\mbox{Binary}$} & \textbf{$\mbox{Multi-class}$} & \textbf{$\mbox{Mixed-type}$}& \textbf{$\mbox{Long-tail}$}\\ %& \textbf{$\mbox{\#IR}$} \\
\hline
{Adult}  & Classification  & 39k/9k   & 'income'        & 3   & 2  & 7  & 2 & 0\\
\hline
  Covertype & Classification& 45k/5k    & 'Cover\_Type'    & 10   & 44 & 1  & 0 & 0\\\hline
 Credit    & Classification& 40k/10k    & 'Class'         & 30  & 1  & 0  & 0 & 1 \\\hline
  Intrusion & Classification& 45k/5k    & 'Class'         & 22   & 6  & 14 & 0 & 2 \\\hline
 Loan     & Classification & 4k/1k       & 'PersonalLoan'  & 5   & 5  & 2  & 1 & 0 \\\hline
 Insurance & Regression &1k/300&'charges'&13&3&2&2&0\\
 \hline
  King & Regression &17.3k/4.3k&'price'&1&6&2&0\\
\hline
% Rad      & 40k/10k       & "Class"  & 22   & 1  & 3  & 1 & 0.28\\
%\multicolumn{5}{l}{%\footnotesize 1. \textbf{$\mbox{\#C}$}: Number of continuous variables } \\
%\multicolumn{5}{l}{\footnotesize 2. \textbf{$\mbox{\#B}$}: Number of binary variables } \\
%\multicolumn{5}{l}{\footnotesize 3. \textbf{$\mbox{\#M}$}: Number of multi-class categorical variables} \\
%\multicolumn{5}{l}{\footnotesize 4. \textbf{$\mbox{\#Bi}$}: Number of \bimodal variables } \\
\end{tabular}
}
\label{table:DD}
\vspace{-0.8em}
\end{table*}

% \subsubsection*{Baselines:} 
{\bf Baselines}. Our \algo is compared with 4 state-of-the-art GAN-based tabular data generators: \ctgan, \tablegan, \cwgan and \medgan. To have a fair comparison, all algorithms are coded using Pytorch, with the generator and discriminator structures matching the descriptions provided in their respective papers. For Gaussian mixture estimation of continuous variables, we use the same settings as the evaluation of \ctgan, i.e. 10  modes. All algorithms are trained for 150 epochs for Adult, Covertype, Credit and Intrusion datasets, whereas the algorithms are trained for 300 epochs on Loan dataset. The reason is Loan dataset is significantly smaller than the others containing only 5000 rows and requires a long training time to converge. %Hence, we believe that the algorithms demand more training to converge. 
Lastly, each experiment is repeated 3 times. %\rb{training epochs for Covertype?}


% \subsubsection{Environment:} 
{\bf Environment}. Experiments are run under Ubuntu 20.04 on a machine equipped with 32 GB memory, a GeForce RTX 2080 Ti GPU and a 10-core Intel i9 CPU.



\subsection{Evaluation Metrics}
\label{sec:metrics}
The evaluation is conducted on three dimensions: (1) machine learning (ML) utility, (2) statistical similarity and (3) privacy preservability. The first two measure if the synthetic data can be used as a good proxy of the original data. The third criterion %sheds light on 
evaluates the nearest neighbour distances within and between the original and synthetic datasets, respectively. 
%The goal is to best maintain the utility and statistical distributions of the original data in the synthetic data, while not memorizing the exact same record as in the original data.
  
\subsubsection{Machine Learning Utility}
\label{sec:ml_efficacy}
% As shown in Fig.~\ref{fig:settingA}, t

To quantify the ML utility, we compare the performance achieved by 5 widely used machine learning algorithms on real versus synthetic data: decision tree classifier, linear support-vector-machine (SVM), random forest classifier, multinomial logistic regression and MLP. 
We use scikit-learn 0.24.2 with default parameters except max-depth 28 for decision tree and random forest, and neurons 128 for MLP.% All other hyper-parameters use their default value.
% If not specified otherwise, we use the default hyper-parameters.
For a fair compassion, all hyper-parameters are fixed across all datasets. Due to this our results can differ slightly from~\cite{ctgan} where the authors use different ML models and hyper-parameters for each dataset. Fig.~\ref{fig:settingA} shows the evaluation process. The train dataset and synthetic dataset are the same size. The aim of this design is to test how close the ML utility is when we train a ML model using the synthetic data vs the real data.

% \ak{Note that for our evaluation, we use the same number of ML models with identical hyper-parameters for each dataset unlike the evaluation performed in the work of \cite{ctgan}.}

% \ak{Details about the hyper-parameters used-:
% For all ML models used, the class weight parameter was set to be "balanced" to take into account the class imbalance in the different datasets. For logistic regression, the default solver i.e "lbfgs"\footnote{http://users.iems.northwestern.edu/~nocedal/lbfgsb.html} and penalty i.e "l2" was used. For the SVM model, the default "rbf" kernel was used with default gamma parameter set to "scale". For both the decision tree  and random forest models, the default "gini" criteria was used and the max depth was set to 28. Lastly, with respect to the MLP model, the "sgd" solver\cite{bottou1991stochastic} was used with a single hidden layer of dimension 128 followed by the default "relu" activation\cite{agarap2018deep}}

% First we split the original data into training and test sets (see Fig.~\ref{fig:settingA}). The training set is used as real data to train the GAN models. Once the training is finished, we use it to
% %use the GAN models to generate synthetic 
% synthesize data with the same size as the training set. The synthetic and real training datasets are then used to train two separate instances of the 5 machine learning models from above. %and evaluated on the real test datasets.
% The ML utility is measured via difference in accuracy, F1-score and area under the ROC between model pairs trained on the real and synthetic data. The aim of this design is to test how close the ML utility is when we train a machine learning model using the synthetic data vs the real data. 

%This responds to the question, ``Can synthetic data be used as a proxy of the original data for training ML models?''. 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.47\columnwidth]{figures/testing_flow_design_correction.png}
%     \caption{Evaluation flows for ML utility}
%     \label{fig:settingA}
%     \vspace{-0.5em}
% \end{figure} 

% \begin{figure}[t]
%   \centering
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{figures/testing_flow_design_correction.png}
%     \caption{Evaluation flows for ML utility}
%       \label{fig:settingA}
%   \end{minipage}
% %   \hfill
%   \begin{minipage}[b]{0.42\textwidth}
%     \label{fig:nndr}
%     \includegraphics[width=\textwidth]{figures/NNDR.png}
%     \caption{Illustration of NNDR}
%   \end{minipage}
%   \vspace{-0.5em}
% \end{figure}



% \begin{figure}[t]
%   \centering
%   \begin{minipage}[b]{0.40\textwidth}
% 	\begin{center}
%         \includegraphics[width=1\columnwidth]{figures/testing_flow_design_correction.png}
%         %\vspace{-1.5em}
% 		\caption{\small{Evaluation for ML utility}}
% 		\label{fig:settingA}
% 	\end{center}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.38\textwidth}
%     %\centering
%     \includegraphics[width=1\columnwidth]{figures/NNDR.png}
%     %\vspace{-1.5em}
%     \caption{Illustration of NNDR}
%     %\vspace{-0.5em}
%     \label{fig:nndr}
%   \end{minipage}
%   %\vspace{-1em}
% \end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.99\columnwidth]{figures/testing_flow_design_correction.png}
    \caption{Evaluation flows for ML utility}
    \label{fig:settingA}
    % \vspace{-0.5em}
\end{figure} 

%     \item \textbf{Setting B}: As shown in Fig.~\ref{fig:settingB}, most of the setting is identical as setting A. The only difference is that after generating data, instead of using synthetic data to train a set of machine learning models, we will merge train dataset and synthetic data together to train the models. The result will be compared with the train dataset only scenario. The aim of this design is to test if the synthetic data can be used as data augmentaion for original data.

% \end{itemize}


\subsubsection{Statistical Similarity}
% \lc{Provide the citation and just mention the key concept. 
% Those are known metrics.}
Three metrics are used to quantify the statistical similarity between real and synthetic data. % they are as follows:

\textbf{Jensen-Shannon divergence (JSD)}. The JSD provides a measure to quantify the difference between the probability mass distributions of individual categorical \columns belonging to the real and synthetic datasets, respectively. Moreover, this metric is bounded between 0 and 1 and is symmetric allowing for an easy interpretation of results. % Note that for each dataset, the distinct JSD values for each categorical column are averaged to obtain a compact comprehensible score.
%Naturally, it is preferred that this final average be as close as 0 as possible to indicate that there is a good match between the probability mass distributions of categorical columns belonging to real and synthetic datasets respectively.

\textbf{Wasserstein distance (WD)}. In similar vein, the Wasserstein distance is used to capture how well the distributions of individual continuous/mixed \columns are emulated by synthetically produced datasets in correspondence to real datasets. 
%The wasserstein distance (a.k.a the earth mover’s distance (EMD)) can be intuitively understood as the minimum amount of “work” required to transform one 1D-probability distribution into another, where the “work” is quantified by the amount of distribution weight that must be moved, multiplied by the distance it has to be moved. As with any distance measure, it is preferred that this distance be as low as possible to signal that the probability distribution of synthetically generated continuous columns is similar to their respective real columns.
%And as was done previously, here too, for each dataset, the distinct distances for each continuous column are averaged to obtain a final score. 
We use WD because we found that the JSD metric was numerically unstable for evaluating the quality of continuous \columns, especially when there is no overlap between the synthetic and original dataset. Hence, we resorted to utilize the more stable Wasserstein distance. 
 %as it often resulted in infinities when values for a continuous column in the synthetic dataset lied outside the range of values in the original dataset. 
 
\textbf{Difference in pair-wise correlation (Diff. Corr.)}. %\lc{The following is very twisty. Be straight and simple. What is the range of this metrics}\lc{Shorten it!!!!} 
To evaluate how well feature interactions are preserved in the synthetic datasets, we first compute the pair-wise correlation matrix for the columns within real and synthetic datasets individually. %To measure the correlation between any two continuous features, the 
Pearson correlation coefficient is used between any two continuous \columns. It ranges between $[-1,+1]$. Similarly, the Theil uncertainty coefficient is used to measure the correlation between any two categorical features. It ranges between $[0,1]$. And the correlation ratio  between categorical and continuous \columns is used. It also ranges between $[0,1]$. Note that the dython\footnote{\url{http://shakedzy.xyz/dython/modules/nominal/\#compute\_associations}} library is used to compute these metrics. Finally, the difference between pair-wise correlation matrices for real and synthetic datasets is computed. 



\subsubsection{Privacy preservability}
To quantify the privacy preservability, we resort to distance metrics (instead of differential privacy (\cite{pategan})) as they are intuitive and easy to understand by data science practitioners. Specifically, we use the following metrics to evaluate the privacy risk.% associated with synthetic datasets.

\textbf{Distance to Closest Record (DCR)}. The DCR is used to measure the Euclidean distance between any synthetic record and its closest corresponding real neighbour. Ideally, the higher the DCR the lesser the risk of privacy breach. Furthermore, the $5^{th}$ percentile of this metric is computed to provide a robust estimate of the privacy risk. % Please note only 5 percent of the data was sampled randomly, stratified on the class label for both real and synthetic data to compute results in a timely manner. 
    
\textbf{Nearest Neighbour Distance Ratio (NNDR)}.
%(\cite{nndr}). %Instead of only measuring the closest neighbour, the 
NNDR measures the ratio between the Euclidean distance for the closest and second closest real neighbour to any corresponding synthetic record. NNDR is a commonly used concept in computer vision area for matching local image descriptors. Platzer\footnote{\url{https://github.com/mostly-ai/virtualdatalab}}  introduces this idea to evaluate the privacy for synthetic data. This ratio is within $[0,1]$. Higher values indicate better privacy. %One can imagine the scenario when we calculate NNDR between real and synthetic dataset. If for our current synthetic data record, the NNDR is extremely small, which means the closest data record in real dataset is far more closer than the second closest data. In that case, the synthetic data and real data composes a small cluster far from other real data, then this 
Low NNDR values between synthetic and real data may reveal sensitive information from the closest real data record. Fig.~\ref{fig:nndr} illustrates the case.  %Hence, this ratio helps to evaluate privacy risk with greater depth and better certainty. 
Note that the $5^{th}$ percentile is computed here as well.% It is ideal for this metric to be low to curtail the risk of privacy. % Please note only 5 percent of the data was sampled randomly, stratified on the class label for both real and synthetic data to compute results in a timely manner.
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.45\columnwidth]{figures/NNDR.png}
%     \caption{Illustration of NNDR metric with its privacy risk implications}
%     \label{fig:nndr}
%     %\vspace{-1em}
% \end{figure} 
%\lc{why do we need two? one is not enough? Add the reason}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/NNDR.png}
    \caption{Illustration of NNDR metric with its privacy risk implications}
    \label{fig:nndr}
    %\vspace{-1em}
\end{figure}
\subsection{Results Analysis}

\begin{figure*}[t]
 	\begin{center}
% 		\subfloat[Adult]{
% 			\includegraphics[width=0.3\textwidth]{figures/Adult.png}
% 			\label{fig:result_adult}
% 		}
% 	\hspace{\fill}
		\subfloat[{Covertype}]{
			\includegraphics[width=0.30\textwidth]{figures/Covtype.jpg}
			\label{fig:result_covtype}
 		}
% 	\hspace{\fill}
% 		\subfloat[Credit]{
% 			\includegraphics[width=0.3\textwidth]{figures/Credit.png}
% 			\label{fig:result_credit}
% 		}
% 	\hspace{\fill}
		\subfloat[{Intrusion}]{
			\includegraphics[width=0.30\textwidth]{figures/Intrusion.jpg}
			\label{fig:result_intrusion}
		}
% 	\quad
		\subfloat[{Loan}]{
			\includegraphics[width=0.30\textwidth]{figures/Loan.jpg}
			\label{fig:result_loan}
		}
		% \vspace{-0.5em}
		\caption{\small{ML utilities difference (i.e., AUC and F1-score) for five algorithms and five datasets}}
		\label{fig:ml_whole}
	\end{center}
	% \vspace{-2em}
\end{figure*}

\textbf{ML Utility}. Tab.~\ref{table:ML_all} shows the average ML utility difference between real and synthetic data in terms of accuracy, F1 score, and AUC. A better synthetic data is expected to have small differences. It can be seen that \algo outperforms all other state-of-the-art methods in terms of Accuracy, F1-score and AUC. Accuracy is the most commonly used classification metric, but since we have imbalanced target \column, F1-score and AUC are more stable metrics for such cases. AUC ranges from 0 to 1. \algo largely shortens the AUC difference from 0.169 (best in state-of-the-art) to 0.094. % \zz{need to update numbers here before submission}  %\lc{Write more about this table. Write the difference among these three. I mean the values themselves! } 

% \begin{table}[t]
% \centering
% \caption{Difference of ML accuracy (\%), F1-score, and AUC between original and synthetic data: average over 5 different datasets and 3 replications.}
% % \resizebox{\columnwidth}{!}{
% % \begin{tabular}{|C{1.7cm}|C{2cm}|C{2cm}|C{2cm}|}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Method} & \textbf{Accuracy} & \textbf{F1-score}  & \textbf{AUC} \\
% \hline
% \small{\algo}    & \textbf{9.83\%} & \textbf{0.127} &   \textbf{0.117}  \\
% \small{CTGAN}    &21.51\% & 0.274 &   0.253 \\
% \small{TableGAN} &11.40\%  & 0.130 &   0.169  \\
% \small{MedGAN}    & 14.11\%&  0.282&   0.285 \\
% \small{CW-GAN}    &  20.06\%& 0.354 &  0.299 \\
% \hline
% \end{tabular}
% % }
% \label{table:ML_all}
% \end{table}

To obtain a better understanding, Fig.~\ref{fig:ml_whole} plots the (F1-score, AUC) for all 5 ML models for the Covertype, Intrusion and Loan datasets. Due to the page limit restrictions, results for Adult and Credit datasets are not shown. Their results are similar to the ones for Covertype (see Fig.~\ref{fig:ml_whole}(a)). %Furthermore, 
Fig.~\ref{fig:ml_whole}(b) shows that for the Intrusion dataset \algo largely outperforms all others across all  ML models used for evaluation. For datasets such as Covertype, the results of \algo and \tablegan are similar and clearly better than the rest. This is because apart from \ctgan, the other models fail to deal with the imbalanced categorical \columns. Furthermore, as \ctgan uses a VGM model with 10 modes, it fails to converge to a suitable optimum for Covertype that mostly comprises single mode Gaussian distributions. %\lc{explaination?}
%\lc{change}For Credit dataset, TableGAN and \algo  show their strength for different ML algorithms, the result of CTGAN is close to above two, but still slightly worse. 

For the Loan dataset (see Fig.~\ref{fig:ml_whole}(c)), \tablegan is better than \algo and others, but the difference between the two is smaller than for the Intrusion dataset. We believe that the reason \algo outperforms the others by such a wide margin (17\% higher than second best for averaged accuracy across the 5 machine learning algorithms) for the Intrusion dataset is that it contains many highly imbalanced categorical \columns. In addition, Intrusion also includes 3 long tail continuous variables. Our results indicate that none of the state-of-the-art techniques can perform well under these conditions. The Loan dataset is significantly smaller than the other four and has the least number of \columns. Moreover, all continuous \columns are either simple one mode Gaussian distributions or just uniform distributions. Therefore, we find that the encoding method in \algo which works well for complex cases, fails to converge to a better optimum for simple and small datasets. %\lc{which one?}

\input{table1_alt}

% \begin{table}[t]
% \centering
% \caption{Statistical similarity: three measures averaged over 5 datasets and three repetitions.}
% % \resizebox{\columnwidth}{!}{
% % \begin{tabular}{|C{1.7cm}|C{2cm}|C{2cm}|C{2cm}|}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Method} & \textbf{Avg JSD} & \textbf{Avg WD}  & \textbf{Diff. Corr.} \\
% \hline
% \small{\algo}   & \textbf{0.0697}&  \textbf{1050}  &  \textbf{2.10} \\
% \small{CTGAN}    & 0.0704&  1769  & 2.73  \\
% \small{TableGAN} & 0.0796& 2117   &  2.30 \\
% \small{MedGAN}   & 0.2135& 46257  &   5.48   \\
% \small{CW-GAN}   & 0.1318& 238155 &  5.82 \\
% \hline
% \end{tabular}
% % }
% \label{table:SS_all}
% \vspace{-0.5em}
% \end{table}

\textbf{Statistical similarity}. Statistical similarity results are reported in Tab.~\ref{table:ML_all}. \algo stands out again across all comparisons. %That indicates that we model the real distribution better than others. 
For categorical \columns (i.e. average JSD), \algo outperforms \ctgan and \tablegan by 13.5\% and 28.4\%. 
%\algo and \ctgan perform similarly (around 0.8\% difference),  %\rb{(within XXX of each other)}, 
%and better than the other methods by at least 12.4\%, i.e. against the next best \tablegan. 
This is due to the use of the conditional vector, the log-frequency sampling and extra losses, which works well for both balanced and imbalanced distributions. For continuous \columns (i.e. average WD), we still benefit from the design of the conditional vector. The average WD column shows some extreme numbers such as 46257 and 238155 comparing to 1197 of \algo. The reason is that these algorithms generate extremely large values for long tail \columns. Besides divergence and distance, our synthetic data also maintains better correlation. We can see that \tablegan also performs well here. However, as the extended conditional vector enhances the training procedure, this helps to maintain even more the correlation between \columns. Because the extended conditional vector allows the generator to produce samples conditioned even on a given VGM mode for continuous \columns. This increases the capacity to learn the conditional distribution for continuous \columns and hence leads to an improvement in the overall feature interactions captured by the model.  %\zz{need to be done}. 
 
 

\textbf{Privacy preservability}. %As only PATE-GAN can generate synthetic data within tight differential privacy guarantees, 
We use distance-based algorithms to give an overview on privacy in our evaluation. On the one hand, if the distance between real and synthetic data is too large, it simply means that the quality of generated data is poor. On the other hand, if the distance between real and synthetic data is too small, it means that there is a risk to reveal sensitive information from the training data. Therefore, the evaluation of privacy is relative. The privacy results are shown in Tab.~\ref{table:ML_all}. It can be seen that the DCR and NNDR between real and synthetic data (i.e., R\&S) all indicate that generation from \tablegan has the shortest distance to real data (i.e., highest privacy risk).
%The algorithm which allows for greater distances between real and synthetic data under equivalent ML utility and statistical similarity data should be considered. 
In that case, \algo not only outperforms \tablegan in ML utility and statistic similarity, but also in all privacy preservability metrics by 11.6\% and 4.5\% for DCR and NNDR, respectively. %\rb{by XXX and XXX for DCR and NNDR, respectively}.
Another insight from this table is that for \medgan, DCR  within synthetic data is 41\% smaller than within real data. This suggests that it suffers from the mode collapse problem.

\input{table2_alt}

% % \lc{Check all captions of all figures and tables..so that it's easy to understand}


% \begin{table}[h]
% \begin{minipage}{.5\linewidth}
%     \centering
%     \caption{Privacy impact.}
%     \label{table:PP_all}
%     \medskip
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{DCR}} & \multicolumn{3}{c|}{\textbf{NNDR}} \\
% \cline{2-7}
%  & \textbf{R\&S} & \textbf{R}  & \textbf{S} & \textbf{R\&S} & \textbf{R}  & \textbf{S}\\

% \hline
% % \algo 2.0 & 1.056 &  0.428& 0.917 & 0.693 & 0.414 &0.570\\
% \algo     & 1.101 &  0.428& 0.877 & 0.714 & 0.414 &0.558\\
% CTGAN    & 1.517 &  0.428& 1.026 & 0.763 & 0.414 &0.624 \\
% TableGAN & 0.988 &  0.428& 0.920 & 0.681 & 0.414 &0.632\\
% MedGAN   & 1.918 &  0.428& 0.254 & 0.871 & 0.414 &0.393 \\
% CW-GAN   & 2.197 &  0.428& 1.124 & 0.847 & 0.414 &0.675\\
% \hline
% \end{tabular}
% }
% % \label{table:ML_all}
% \end{minipage}\hfill
% \begin{minipage}{.5\linewidth}
%     \centering
%     \caption{F1-score difference to CTAB-GAN}
%     % \label{tab:second_table}
%     \medskip
%     \resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{ |C{1.8cm}|C{1.4cm}|C{1.2cm}|C{2.2cm}| C{1.5cm}|}
% \hline
% \textbf{Dataset} & \textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM and Mode vector}& \textbf{\algo} \\
% %\textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
% \hline
%  %-0.018&	-0.161& -0.018 &-0.01 & 0.704  \\
% % \hline
% Adult &  -0.01&	-0.037 & -0.05  & 0.704  \\
% \hline
% Covertype & -0.018 & -0.184& -0.118  & 0.532\\
% \hline
% Credit & +0.011& -0.177& +0.06&  0.71 \\
% \hline
% Intrusion &-0.031&-0.437&+0.003& 0.842 \\
% \hline
% Loan &-0.044&+0.028&+0.013  & 0.803 \\
% \hline
% \end{tabular}
% }
% \label{table:ablation}
% \end{minipage}
% \vspace{-1em}
% \end{table}





% \begin{table}[t]
% \centering
% \caption{Privacy impact: between real and synthetic data (R\&S) and within real data (R) and synthetic data (S).}
% % \resizebox{\columnwidth}{!}{
% % \begin{tabular}{ |C{2cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|C{1.5cm}|}
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{DCR}} & \multicolumn{3}{c|}{\textbf{NNDR}} \\
% \cline{2-7}
%  & \textbf{R\&S} & \textbf{R}  & \textbf{S} & \textbf{R\&S} & \textbf{R}  & \textbf{S}\\

% \hline
% % \algo 2.0 & 1.056 &  0.428& 0.917 & 0.693 & 0.414 &0.570\\
% \algo     & 1.101 &  0.428& 0.877 & 0.714 & 0.414 &0.558\\
% CTGAN    & 1.517 &  0.428& 1.026 & 0.763 & 0.414 &0.624 \\
% TableGAN & 0.988 &  0.428& 0.920 & 0.681 & 0.414 &0.632\\
% MedGAN   & 1.918 &  0.428& 0.254 & 0.871 & 0.414 &0.393 \\
% CW-GAN   & 2.197 &  0.428& 1.124 & 0.847 & 0.414 &0.675\\
% \hline
% \end{tabular}
% % }
% \label{table:PP_all}
% \end{table}


% \begin{table}[t]
% \begin{minipage}{.5\linewidth}
%     \centering
%     \caption{Privacy impact.}
%     \label{table:PP_all}
%     \medskip
% \resizebox{1\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{DCR}} & \multicolumn{3}{c|}{\textbf{NNDR}} \\
% \cline{2-7}
%  & \textbf{R\&S} & \textbf{R}  & \textbf{S} & \textbf{R\&S} & \textbf{R}  & \textbf{S}\\

% \hline
% % \algo 2.0 & 1.056 &  0.428& 0.917 & 0.693 & 0.414 &0.570\\
% \algo     & 1.101 &  0.428& 0.877 & 0.714 & 0.414 &0.558\\
% CTGAN    & 1.517 &  0.428& 1.026 & 0.763 & 0.414 &0.624 \\
% TableGAN & 0.988 &  0.428& 0.920 & 0.681 & 0.414 &0.632\\
% MedGAN   & 1.918 &  0.428& 0.254 & 0.871 & 0.414 &0.393 \\
% CW-GAN   & 2.197 &  0.428& 1.124 & 0.847 & 0.414 &0.675\\
% \hline
% \end{tabular}
% }
% % \label{table:ML_all}
% \end{minipage}\hfill
% \begin{minipage}{.5\linewidth}
%     \centering
%     \caption{F1-score difference to CTAB-GAN}
%     % \label{tab:second_table}
%     \medskip
%     \resizebox{0.9\columnwidth}{!}{
% \begin{tabular}{ |C{1.8cm}|C{1.4cm}|C{1.2cm}|C{2.2cm}| C{1.5cm}|}
% \hline
% \textbf{Dataset} & \textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM and Mode vector}& \textbf{\algo} \\
% %\textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
% \hline
%  %-0.018&	-0.161& -0.018 &-0.01 & 0.704  \\
% % \hline
% Adult &  -0.01&	-0.037 & -0.05  & 0.704  \\
% \hline
% Covertype & -0.018 & -0.184& -0.118  & 0.532\\
% \hline
% Credit & +0.011& -0.177& +0.06&  0.71 \\
% \hline
% Intrusion &-0.031&-0.437&+0.003& 0.842 \\
% \hline
% Loan &-0.044&+0.028&+0.013  & 0.803 \\
% \hline
% \end{tabular}
% }
% \label{table:ablation}
% \end{minipage}
% \vspace{-1em}
% \end{table} 
\subsection{Ablation Analysis}
To illustrate the efficiency of each strategy we implement an ablation study which cuts off the different components of \algo one by one: (1) \textbf{w/o $\mathcal{C}$}. In this experiment, Classifier $\mathcal{C}$ and the corresponding classification loss for Generator $\mathcal{G}$ are taken away from \algo; (2) \textbf{w/o I. loss} (information loss). In this experiment, we remove information loss from \algo; (3) \textbf{w/o MSN}. In this case, we substitute the mode specific normalization based on VGM for continuous \columns with min-max normalization and use simple one-hot encoding for categorical \columns. Here the conditional vector is the same as for \ctgan; (4) \textbf{w/o LT} (long tail). In this experiment, long tail treatment is no longer applied. This only affects datasets with long tailed columns, i.e. Credit and Intrusion.

% , instead of using variational Gaussian Mixture model, we simply use min and max value to normalize each value in the \column, and each value is encoded as a scalar indicating the value in the row vector. Since we do not use VGM in that case, there thus is no more mode of Gaussian mixture. The conditional vector becomes the same format as in CTGAN.

% \textbf{w/o Mode vector} In that case, our objective is to compare with the conditional vector in CTGAN. The conditional vector CTGAN only allows to choose the class of categorical column, not for individual mode in continuous or mix data type columns. Therefore, this result will show the effect of adding modes information from continuous column into conditional vector. 
%\lc{Repeat again the average of 5 ML}
The results are compared with the baseline implementing all strategies. 
All experiments are repeated 3 times, and results are evaluated on the same 5 machine learning algorithms introduced in Sec.~\ref{sec:ml_efficacy}. 
%We report the F1-score difference between \algo and each above-mentioned experiments,  
The test datasets and evaluation flow are the same as shown in Sec.~\ref{ssec:setup} and Sec.~\ref{sec:metrics}. %, and all the experiments are repeated 3 times.
Tab.~\ref{table:ablation_and_timing} shows the results.
Each part of \algo has different impacts on different datasets. For instance, \textbf{w/o $\mathcal{C}$} has a negative impact for all datasets except Credit.
Since Credit has only 30 continuous \columns and one target \column, the semantic check can not be very effective.
\textbf{w/o information loss} has a positive impact for Loan, but results degenerate for all other datasets. It can even make the model unusable, e.g. for Intrusion. \textbf{w/o MSN} performs bad for Covertype, but has little impact for Intrusion. Credit w/o MSN performs  better than original \algo. This is because out of 30 continuous \columns, 28 are nearly single mode Gaussian distributed. The initialized high number of modes, i.e. 10, for each continuous \column (same setting as in \ctgan) degrades the estimation quality. \textbf{w/o LT} has the biggest impact on Intrusion, since it contains 2 long tail columns which are important predictors for the target column. For Credit, the  influence is limited. Even if the long tail treatment fits well the \textit{amount} column (see Sec.~\ref{sec:further}), this variable is not a strong predictor for the target column.
%We can observe the similar result for CTGAN under Covertype datasets which is shown in Fig.~\ref{fig:result_covtype}. Because Covertype has a similar distribution for all continuous \column as Credit.
In general, if we average the column values, all the ablation tests have a negative impact for the performance which justifies our design choices for \algo. 

% \begin{table}[t]
% \centering
% \caption{F1-score difference to \algo. \algo column reports the absolute averaged F1-score as baseline.}
% \label{table:ablation}
% \resizebox{0.5\columnwidth}{!}{
% \begin{tabular}{ |C{1.8cm}|C{1.4cm}|C{1.2cm}|C{2.2cm}| C{1.5cm}|}
% \hline
% \textbf{Dataset} & \textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM and Mode vector}& \textbf{\algo} \\
% %\textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
% \hline
%  %-0.018&	-0.161& -0.018 &-0.01 & 0.704  \\
% % \hline
% Adult &  -0.01&	-0.037 & -0.05  & 0.704  \\
% \hline
% Covertype & -0.018 & -0.184& -0.118  & 0.532\\
% \hline
% Credit & +0.011& -0.177& +0.06&  0.71 \\
% \hline
% Intrusion &-0.031&-0.437&+0.003& 0.842 \\
% \hline
% Loan &-0.044&+0.028&+0.013  & 0.803 \\
% \hline
% \end{tabular}
% }
% \end{table}

% \begin{table}[t]
% \centering
% \caption{F1-score difference to \algo. \algo column reports the absolute averaged F1-score as baseline.}
% \label{table:ablation}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{ |C{1.4cm}|C{1.4cm}|C{1.2cm}|C{1.5cm}| C{1.5cm}|}
% \hline
% \textbf{Dataset} & \textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
% %\textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
% \hline
%  %-0.018&	-0.161& -0.018 &-0.01 & 0.704  \\
% % \hline
% Adult &  -0.01&	-0.037 & -0.05 &+0.08 & 0.704  \\
% \hline
% Covertype & -0.018 & -0.184& -0.118 &-0.077 & 0.532\\
% \hline
% Credit & +0.011& -0.177& +0.06& -0.051 & 0.71 \\
% \hline
% Intrusion &-0.031&-0.437&+0.003& +0.019 & 0.842 \\
% \hline
% Loan &-0.044&+0.028&+0.013&0  & 0.803 \\
% \hline
% \end{tabular}
% }
% \end{table}



% \begin{table*}[t]
% \centering
% \caption{Ablation and Training Time Analysis For \algoplus}
% \label{}
% \resizebox{1.0\textwidth}{!}{
% \begin{tabular}{|c||c|c|c|c|c||c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{5}{c||}{\bf Ablation [F1 score]} &
% \multicolumn{5}{c|}{\bf Training Time [s/epoch]} \\
% \cline{2-11}
%  & \textbf{\algo} & \textbf{w/o $\mathcal{C}$} & \textbf{w/o I. Loss}  & \textbf{w/o MSN} & \textbf{w/o LT} & 
% \textbf{{\algoplus}} &\textbf{{\ctgan}} & \textbf{{\tablegan}}  & \textbf{{\medgan}} & \textbf{{\cwgan}} \\
% %\textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
% \hline
%  %-0.018&	-0.161& -0.018 &-0.01 & 0.704  \\
% % \hline
% Adult &  &  & &  &   &    &       &    &   &  \\
% % \hline
% Covertype  &  &  & &  &   &    &       &    &   &   \\
% % \hline
% Credit &  &  & &  &   &    &       &    &   &  \\
% % \hline
% Intrusion &  &  & &  &   &    &       &    &   &  \\
% % \hline
% Loan &  &  & &  &   &    &       &    &   &  \\
% Insurance &  &  & &  &   &    &       &    &   &\\

% \hline
% \end{tabular}
% }
% \label{table:ablation_and_timing_algoplus}
% %\vspace{-1em}
% \end{table*}




% \begin{table}[t]
% \centering
% \caption{Training time per epoch.}
% \resizebox{0.7\columnwidth}{!}{
% \begin{tabular}{ |C{2cm}|C{2.4cm}|C{1.8cm}|C{2cm}|C{1.8cm}|C{1.8cm}|C{1.8cm}| }
% \hline
% \textbf{Dataset} & \textbf{\small{\algo}} &\textbf{\small{\ctgan}} & \textbf{\small{\tablegan}}  & \textbf{\small{\medgan}} & \textbf{\small{\cwgan}}\\ 
% \hline
% \small{Adult}     & 7.50   &1.66       & 0.52   & 0.33  & 4.73  \\
% \hline
%  \small Covertype & 8.38    &3.32    & 1.69   & 0.33 & 10.41   \\\hline
% \small Credit    & 8.92    &2.42         & 1.73  & 0.34  & 4.50  \\ 
% \hline
%  \small Intrusion & 10.73    &2.80        & 1.75   & 0.34  & 10.81  \\\hline
% \small Loan      & 0.57   &0.17        & 0.06   & 0.04  & 1.12  \\
% \hline
% \end{tabular}
% }
% \label{table:training_time}
% \vspace{-0.8em}
% \end{table}
% \subsection{Further discussion}
% \label{sec:further}

\subsection{Training Time Analysis}
%\rb{what about inference time? are we also significantly slower? if not it would make sense to include those results and argue that for offline training online infercne use cases we are still good} 
The above results show that \algo outperforms the State of the art in ML utility, statistical similarity and privacy preservation. This comes at the expense of additional training complexity, i.e., information, classifier and generator losses, and feature encoding, i.e., mixted-type, long tail, and VGM mode in conditional vectors. %which translates into longer training times.
Tab.~\ref{table:ablation_and_timing} shows the training time per epoch for all models on all datasets. As expected, \algo is slower than other algorithms. To improve the training efficiency of \algo, we may do the following: (1) 
%instead of training the classifier together with the generator for each epoch, we can
pre-train the classifier with the real dataset before-hand instead as in parallel to the generator. By storing once the inference results we can speed up the calculation of the classifier loss. 
%\rb{check if correct} \rb{should this maybe not help also in convergence? (i.e. the classifier loss might not be very reliable at the beginning?)}
%We thus cut the training time for updating the generator via the classifier loss; 
(2) use min-max normalization instead of a VGM estimation for continuous columns with a clear single mode Gaussian distribution. Since VGM estimates $k >> 1$ modes, using min-max normalization can significantly reduce the length of the continuous column encoding; (3) treat categorical columns with a clear single mode Gaussian distribution as a continuous column and use min-max normalization instead of one-hot encoding. To convert values back to categorical form, rounding has been shown to work well in \cite{tablegan}. (1) is easy to adopt. However, (2) and (3) require human intuition to verify and determine the distribution of each column before training. From our preliminary study based on Adult dataset, \algo can reduce training time by 29\% implementing (1) and by 12\% using (2) and (3) while maintaining a similar quality of generation.
%\rb{for 2 and 3 could you not do some statistical tests?} \rb{justify why not 1 already implemented}}
%Fundamentally, capturing the complexity of a probability distribution in it's most simple form with the least number of parameters to know if we need VGM or not is quite difficult for the VGM algorithm as likelihood based estimation favours greater number of parameters. But it is very simple for a human by just looking at the visual representation of the distribution.

% \input{table3}




\subsection{Results for Motivation Cases}
\label{sec:further}


\begin{figure*}[ht]
	\begin{center}
	
		\subfloat[\textit{bmi} in Insurrance]{
			\includegraphics[width=0.25\textwidth]{figures/single_gaussian_ctabgan.png}
			\label{fig:ctabgan_single_gaussian}
		}
		\subfloat[\textit{Mortgage} in Loan]{
			\includegraphics[width=0.25\textwidth]{figures/bimodal_ctabgan_update.png}
			\label{fig:ctabgan_bimodal}
		}
% 			\hspace{\fill}
		\subfloat[\textit{Amount} in Credit]{
			\includegraphics[width=0.22\textwidth]{figures/result_longtail.png}
			\label{fig:longtail_result}
		}
				% 	\hspace{\fill}
		\subfloat[\textit{Hours-per-week} in Adult]{
			\includegraphics[width=0.245\textwidth]{figures/result_gmm.png}
			\label{fig:gmm_result}
		}
		\caption{ Challenges of modeling industrial dataset using existing GAN-based table generator: (a)simple gaussian (b) \bimodal type, (c) long tail distribution, and (d) \skewed data} %\zz{count to pdf, density to cdf.}}
		\label{fig:motivationcases_response}
 	\end{center}
\end{figure*}


After reviewing all the metrics, let us recall the three motivation cases from Sec.~\ref{sec:motivation}. 

{\bf \Mixed data type \variables}. Fig.~\ref{fig:motivationcases_response}(a) compares the real and \algo generated \column \textit{Mortgage} in Loan dataset. \algo encodes this \column as \bimodal type. We can see that \algo generates clear 0 values and the frequency is close to real data. %One drawback which can be observed is that \algo amplifies the dominance of the 0 in this \column. Even with our log-frequency-based sampling of Gaussian mixture modes and categorical classes, \algo generates more 0 values than in the original distribution. That means there is still room for improvement for extremely imbalanced cases. 
%\subsubsection{Mix-type encoder}
% \begin{figure}[htb]
% 	\begin{center}
% 		\subfloat[Real]{
% 			\includegraphics[width=0.45\columnwidth]{figures/bimodal_original.png}
% 			\label{fig:real_bimodal}
% 		}
% 	    \hspace{\fill}
% 		\subfloat[\algo]{
% 			\includegraphics[width=0.45\columnwidth]{figures/bimodal_ctabgan.png}
% 			\label{fig:ctabgan_bimodal}
% 		}
%  		\caption{Generation for \bimodal column \textit{Mortgage} in Loan dataset}
%  		\label{fig:ctabgan_bimodal}
% 	\end{center}
% \end{figure}

{\bf Long tail distributions.} Fig.~\ref{fig:motivationcases_response}(b) compares the cumulative frequency graph for the \textit{Amount} \column in Credit. This \column is a typical long tail distribution. %According to Fig.~\ref{fig:real_longtail}, %most of the occurrences are gathered near the head of distribution, but the end of distribution is near 25 000. 
One can see that \algo perfectly recovers the real distribution. Due to log-transform data pre-processsing, \algo learns this structure significantly better than the state-of-the-art methods shown in Fig.~\ref{fig:motivationcases}(b).  %which is proposed Eq.\eqref{eq:preprossesing}. 
% TableGAN models well the structure at the beginning, but the distribution stops at around 6000. Other algorithms fail to model this column.
% \begin{figure}[htb]
% 	\begin{center}
% 		\subfloat[Real]{
% 			\includegraphics[width=0.45\columnwidth]{figures/real_longtail.png}
% 			\label{fig:real_longtail}
% 		}
% 			\hspace{\fill}
% 		\subfloat[\algo]{
% 			\includegraphics[width=0.45\columnwidth]{figures/ctabgan_longtail.png}
% 			\label{fig:ctabgan_longtail}
% 		}
% 		\caption{Cumulative frequency graph of generation for \textit{Amount} column in Credit dataset}
% 		\label{fig:longtail_result}
% 	\end{center}
% \end{figure}

% {\bf Effectiveness of conditional vector}.
{\bf \Skewed multi-mode continuous \variables}.
Fig.~\ref{fig:motivationcases_response}(c) compares the frequency distribution for the continuous \column \textit{Hours-per-week} from Adult. Except the dominant peak at 40, there are many side peaks. Fig.~\ref{fig:motivationcases}(c), shows that \tablegan, \cwgan and \medgan struggle since they can learn only a simple Gaussian distribution due to the lack of any special treatment for continuous \columns. \ctgan, which also use VGM, can detect other modes. Still, \ctgan is not as good as \algo. The reason is that \ctgan lacks the mode of continuous \columns in the conditional vector. By incorporating the  mode of continuous \columns into conditional vector, we can apply the training-by-sample and logarithm frequency also to modes. This gives the mode with less weight more chance to appear in the training and avoids the mode collapse. 
%which generates data only around one or two mode.
% \begin{figure}[htb]
% 	\begin{center}
% 		\subfloat[Real]{
% 			\includegraphics[width=0.45\columnwidth]{figures/real_gmm.png}
% 			\label{fig:real_gmm}
% 		}
% 			\hspace{\fill}
% 		\subfloat[\algo]{
% 			\includegraphics[width=0.45\columnwidth]{figures/ctabgan_gmm.png}
% 			\label{fig:ctabgan_gmm}
% 		}
%  		\caption{Generation for continuous column \textit{Hours-per-week} in Adult dataset}
%  		\label{fig:gmm_result}
%  	\end{center}
% \end{figure}



% \begin{figure*}[htb]
% 	\begin{center}
% 		\subfloat[Real]{
% 			\includegraphics[width=0.33\textwidth]{figures/result_bimodal.png}
% 			\label{fig:ctabgan_bimodal}
% 		}

% 		\subfloat[\algo]{
% 			\includegraphics[width=0.33\textwidth]{figures/result_longtail.png}
% 			\label{fig:longtail_result}
% 		}
		
% 		\subfloat[\algo]{
% 			\includegraphics[width=0.33\textwidth]{figures/result_gmm.png}
% 			\label{fig:gmm_result}
% 		}
%  		\caption{Generation for continuous column \textit{Hours-per-week} in Adult dataset}
%  		\label{fig:response_motivation}
%  	\end{center}
% \end{figure*}


% \begin{figure*}[t]
% 	\begin{center}
% 		\subfloat[Mortgage in Loan]{
% 			\includegraphics[width=0.33\textwidth]{figures/result_bimodal.png}
% 			\label{fig:ctabgan_bimodal}
% 		}
% % 			\hspace{\fill}
% 		\subfloat[Amount in Credit]{
% 			\includegraphics[width=0.31\textwidth]{figures/result_longtail.png}
% 			\label{fig:longtail_result}
% 		}
% 				% 	\hspace{\fill}
% 		\subfloat[Hours-per-week in Adult]{
% 			\includegraphics[width=0.335\textwidth]{figures/result_gmm.png}
% 			\label{fig:gmm_result}
% 		}
% 		\caption{ Challenges of modeling industrial dataset using existing GAN-based table generator: (a) \bimodal type, (b) long tail distribution, and (c) \imbalanced data.} %\zz{count to pdf, density to cdf.}}
% 		\label{fig:motivationcases_response}
%  	\end{center}
% \end{figure*}



==> introduction.tex <==
\section{Introduction}

``Data is the new oil'' is a quote that goes back to 2006, which is credited to mathematician Clive Humby. It has recently picked up more steam after The Economist\footnote{\url{https://www.economist.com/leaders/2017/05/06/the-worlds-most-valuable-resource-is-no-longer-oil-but-data}} published a report titled ``The world's most valuable resource is no longer oil, but data''. Many companies nowadays discover valuable business insights from various internal and external data sources. However, the big knowledge behind big data often impedes personal privacy and leads to unjustified analysis (\cite{narayanan2008}).  To prevent the abuse of data and the risks of privacy breaching, the European Commission introduced the European General Data Protection Regulation (GDPR)  and enforced strict data protection measures. This however instills a new challenge in the data-driven industries to look for new scientific solutions that can empower big discovery while respecting the constraints of data privacy and governmental regulation.  

An emerging solution is to leverage synthetic data (\cite{cramergan}), which statistically resembles real data and can comply with GDPR due to its synthetic nature. The industrial datasets (at stakeholders like banks,  insurance companies, and health care) present multi-fold challenges. First of all, such datasets are organized in tables and populated with both continuous and categorical variables, or a mix of the two, e.g., the value of mortgage for a loan holder. This value can be either 0 (no mortgage) or some continuous positive number. Here, we term such a type of \variables, \textbf{\mixed \variable}.  Secondly data \variables often have a wide range of values as well as skewed frequency distribution, e.g., the statistic of transaction amount for credit card. Most transactions should be within 0 and 500 bucks (i.e. daily shopping for food and clothes), but exceptions of a high transaction amount surely exist.

Generative Adversarial Network (GAN) (\cite{gan}) is one of the emerging data synthesizing methodologies. The GAN is first trained on a real dataset. Then used to generate data. 
%relatively small ``real'' dataset. Then used to generate data.
Beyond its success on generating images, 
%GAN has recently been applied to generate tabular data~
\cite{ctgan, tablegan, cramergan} have recently applied GAN to generate tabular data. The state of the art of tabular generator (\cite{ctgan}) treats categorical variables via conditional GAN, where each categorical value is considered as a condition. However, their focus is only on two types of variables, namely continuous and categorical, overlooking an important class of \mixed data type. In addition, it is unclear if existing solutions can efficiently handle highly \imbalanced categorical variables and skewed continuous variables.

% In this paper, we aim to design a tabular data synthesizer that addresses the limitations of the prior stat-of-the-art: (i) encoding \mixed data type of continuous and categorical variables, (ii) efficient modeling of \imbalanced and long tail variables of all three data types. We propose a novel conditional table geneerative adversarial network, \algo. Two key features of \algo are the introduction of classifier loss in conditional GAN, and novel encoding for the conditional vector that efficiently encodes mixed variables and \imbalanced data distribution per variable.

In this paper, we aim to design a tabular data synthesizer that addresses the limitations of the prior state-of-the-art: (i) encoding \mixed data type of continuous and categorical variables, (ii) efficient modeling of long tail continuous variables and (iii) increased robustness to \imbalanced categorical \variables along with skewed continuous \variables. Hence, we propose a novel conditional table generative adversarial network, \algo. Two key features of \algo are the introduction of classification loss in conditional GAN, and novel encoding for the conditional vector that efficiently encodes mixed variables and helps to deal with highly skewed distributions for continuous variables.


%which using convolutional neural networks (CNN) as generator and discriminator. 

% \begin{shaded*}
%     \textit{\textbf{RQ1}: How to model the mixed data type of continuous and discrete variables? }
% \end{shaded*}

% \begin{shaded*}
%     \textit{\textbf{RQ2}: How to solve the data \imbalanced issues for all data types?
%     }
% \end{shaded*}
%By using \bimodal, we also solved the problem for dataset with empty cells, as we transfer the empty cells as one type of categorical variable.

% \begin{figure}[htp]
% \begin{center}
% \includegraphics[width=0.5\textwidth]{spiral.eps}
% \caption{A spiral.}\label{fig:spiral}
% \end{center}
% \end{figure}

% \begin{figure}[htbp]
%   \subfigure{\includegraphics{figures/bimodal_motivation_case_new}}
%   \subfigure{\includegraphics{figures/merge_image-2}}
% \end{figure}

% \begin{figure}
%         \begin{subfigure}[b]{0.25\textwidth}
%                 \includegraphics[width=\linewidth]{figures/bimodal_motivation_case_new.png}
%                 \caption{A gull}
%                 \label{fig:gull}
%         \end{subfigure}%
%         \begin{subfigure}[b]{0.25\textwidth}
%                 \includegraphics[width=\linewidth]{figures/merge_image-2.png}
%                 \caption{A gull2}
%                 \label{fig:gull2}
%         \end{subfigure}%
%         \caption{Pictures of animals}\label{fig:animals}
% \end{figure}
% \begin{figure}[t]
% \floatconts
%   {fig:subfigex}
%   {\caption{Challenges of modeling industrial dataset using existing GAN-based table generator: (a) \bimodal type, (b) long tail distribution, and (c) \skewed data}}
%   {%
%     \subfigure[\small{Mortgage in Loan dataset}]{\label{fig:mortgage_column_motivation}%
%       \includegraphics[width=0.325\linewidth]{figures/bimodal_motivation_case_new.png}}%
%      \subfigure[\small{Amount in Credit dataset}]{
% 			\includegraphics[width=0.295\textwidth]{figures/merge_image-2.png}
% 			\label{fig:amount_result_motivation}
% 		}
% 	  \subfigure[\footnotesize{Hours-per-week in Adult dataset}]{
% 			\includegraphics[width=0.33\textwidth]{figures/extended_condvec_motivation_case.png}
% 			\label{fig:gmm_result_motivation}
% 		}
%   }
%   \label{fig:motivationcases}
%   \vspace{-1.5em}
% \end{figure}


\begin{figure*}[t]
	\begin{center}
		\subfloat[\textit{bmi} in Insurance]{
			\includegraphics[width=0.25\textwidth]{figures/general_transformer_motivation.png}
			\label{fig:bmi_column_motivation}
		}
		\subfloat[\textit{Mortgage} in Loan]{
			\includegraphics[width=0.25\textwidth]{figures/bimodal_motivation_case_new.png}
			\label{fig:mortgage_column_motivation}
		}
		\subfloat[\textit{Amount} in Credit]{
			\includegraphics[width=0.22\textwidth]{figures/merge_image-2.png}
			\label{fig:amount_result_motivation}
		}
		\subfloat[\textit{Hours-per-week} in Adult]{
			\includegraphics[width=0.25\textwidth]{figures/extended_condvec_motivation_case.png}
			\label{fig:gmm_result_motivation}
		}
% 		\vspace{-0.5em}
		\caption{ Challenges of modeling industrial dataset using existing GAN-based table generator: (a) simple gaussian (b) \bimodal type, (c) long tail distribution, and (d) \skewed data} 
		\label{fig:motivationcases}
 	\end{center}
% \vspace{-2em}
\end{figure*}


We rigorously evaluate \algo in three dimensions: (i) utility of machine learning based analysis on the synthetic data, (ii) statistical similarity to the real data, and (iii) privacy preservability.
Specifically, the proposed \algo is tested on 5 widely used machine learning datasets: Adult, Covertype, Credit, Intrusion and Loan, against 4 state-of-the-art GAN-based tabular data generation algorithms: \ctgan, \tablegan, \cwgan and \medgan. Our results show that \algo not only outperforms all the comparisons in machine learning utility and statistical similarity but also provides better distance-based privacy guarantees than \tablegan, the second best performing algorithm in the machine learning utility and statistical similarly evaluation.
 
The main contributions of this study can be summarized as follows: (1) Novel conditional adversarial network which introduces a classifier providing additional supervision to improve its utility for ML applications. (2) Efficient modelling of continuous, categorical, and \textbf{\bimodal} variables via novel data encoding and conditional vector. (3) Light-weight data pre-processing to mitigate the impact of long tail distribution of continuous variables. (4) Providing an effective data synthesizer for the relevant stakeholders.
% \begin{itemize}[noitemsep]
%  \item Novel conditional adversarial network which introduces a classifier providing additional supervision to improve its utility for ML applications. % via information and classifier loss. % in our model, we adopt a lot of great ideas from previous researches. For example, \textit{Information Loss} and \textit{Classification Loss} from TableGAN. Conditional vector and Variational Gaussian Mixture (VGM) estimation for continuous column from CTGAN. But we do not stop at this step, we extend the original idea. For instance, we design the convolutional neural network (CNN) for Generator and Discriminator, and Multi-Layer Perceptron (MLP) for classifier. We also extend the conditional vector with VGM modes. More details are given in Section~\ref{sec:design_algorithm}. \lc{elaborate}
%  \item Efficient modelling of continuous, categorical, and \textbf{\bimodal} variables via novel data encoding and conditional vector.
%  \item Light-weight data pre-processing to mitigate the impact of long tail distribution of continuous variables. 
%  \item Providing an effective data synthesizer for the relevant stakeholders.
%  \textbf{mix-type encoder}: 
%  to solve the  mix data type in one column and missing value problems, \textbf{\bimodal} and \textbf{mix-type encoder} are proposed to properly represent this kind of column.
%  \item New design for conditional vector: combine categorical encoding with the encoding of mode from Gaussian mixture estimation. % Since we sample the real data according to conditional vector, and 
%  We construct the conditional vector by probability based on logarithm frequency of occurrences of each class from categorical column and each mode from continuous or \bimodal column. Therefore, our training will give more chance to minority class and mode in these columns, improve the problem of mode collapse when training on imbalanced dataset.
%  \item Improving results in long-tailed distribution column: for most of case in continuous column, Gaussian mixture model can estimate well the distribution. But apparently, it is not suitable for long-tailed distribution. Therefore, we propose a pre-processing step to conduct a logarithm transformation for this kind column. 
%\end{itemize}


 

==> model_v2.tex <==
\section{\algoplus}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/ctabplus_diagram.png}
    %\vspace{-1em}
    \caption{\zz{Synthetic Tabular Data Generation via \algoplus}}
    \label{fig:STD}
   %\vspace{-1em}
\end{figure*}
\zz{
\algoplus is a tabular data generator designed to overcome the challenges outlined in Sec.~\ref{sec:motivation}. In \algo we invent a \textit{\encoder} which can better represent mixed categorical-continuous variables as well as missing values. \algo is based on a conditional GAN (CGAN) to efficiently treat minority classes, with the addition of classification, information and generator loss (\cite{tablegan,acgan,ctgan}) to improve semantic integrity and training stability, respectively. Finally, we leverage a log-frequency sampler to overcome the mode collapse problem for imbalanced \columns.} 

\ifshowntationtable
Before illustrating \algo, we summarized the used notation in Table~\ref{tab:symboltable}.

\begin{table}
\centering
\caption{Notation}
\label{tab:symboltable}
\begin{tabular}{|C{1.5cm} |L{6cm}|} \hline
\textbf{Symbol}	& \textbf{Description}\\ \hline
$\mathcal{G}$	& Generator of \algo					 \\\hline
$\mathcal{D}$ 	& Discriminator of \algo					 \\\hline
$\mathcal{C}$	& Classifier of \algo					 \\\hline
% $\mathfrak{L}_{in}$	& Information Loss					 \\\hline
% $\mathfrak{L}^Y_{X}$ & Loss of dataset Y calculated on model X				 \\\hline
$\mathcal{V}$	& Conditional vector %where the mode or categorical vector for column j, the $k$th bit set to 1	 
\\\hline
% $C_j$ 	& Column j					 \\\hline
$\mathcal{N}$ 	& Normal distribution					 \\\hline
$\mu_i$ 	& value of categorical mode, mean value of Gaussian mixture mode					 \\\hline
$\rho_i$ 	& probability density calculated based on mode $i$					 \\\hline
$\gamma_{i,j}$&  one-hot encoding vector for $i$th row value in categorical \column $j$			\\\hline
$\bigoplus$&  vector concatenation			\\\hline
\end{tabular}
\end{table}
\fi

% We use:
% 1) a conditional GAN base architecture to ....
% 2) an auxiliary classifier provided loss feedback to ...improve stability and semantic integrity. 
% 3) a novel data encoder for mixed type variables to ... value plus mode indicator (mode integrated into conditional vector)
% 4) a log-frequency sampler to address the problem of unbalanced datasets.

% variatonal gausssian mixture 

% conditional GAN: added conditional vector to efficiently generate data for minority classes. 
% classifier: to improve semantic integrety

% novel encoder: mixed type and missing values

% log-frequency sampling: used to construct the conditional vectors

% TableGAN: use classsifier, but normal GAN (not conditional GAN) idea from ACGAN
% - information loss: mean + std of generated vs original data (for whole dataset) works well since most columns are normal distributed (term in loss function to train generator)
% CTGAN: uses conditional GAN but no classifier


% Design:
% what loss? Is it important that G and D are CNN while C is MLP?

% \algo is a conditional GAN based method. In \algo, we invent a \textit{Mix-Type Encoder} to model tabular data, which can better represent categorical, continuous and missing values.  We also introduce an strategy which leverages our designed conditional vectors to overcome the mode collapse problem for imbalanced mode columns. \algo also introduces the information loss~\cite{tablegan} and classifier into the CGAN structure to improve the stability of GAN enhance the ability for semantic integrity. Before illustrate the method, all used symbols are summarized in Table~\ref{tab:symboltable}.



\subsection{Technical Background}

\subsubsection{Tabular GAN}
\zz{
GANs are a popular method to generate synthetic data first applied with great success to images~\cite{stylegan} and later adapted to tabular data~\cite{yahi_gan}. GANs leverage an adversarial game between a generator trying to synthesize realistic data and a discriminator trying to discern synthetic from real samples.}

To address the problem of dataset imbalance, we leverage \textit{conditional generator} and \textit{training-by-sampling} methods from CTGAN. The idea behind this is to use an additional vector, termed as the conditional vector, to represent the classes of categorical \columns. This vector is both fed to the generator and used to bound the sampling of the real training data to subsets satisfying the condition. We can leverage the condition to resample all classes giving higher chances to minority classes to train the model. %CTGAN also proposes to use Gaussian mixture estimation for continuous column, which helps to better represent the continuous column of complex distribution.

To enhance the generation quality, we incorporate three extra terms in the loss function of the generator: information (\cite{tablegan}), classification (\cite{acgan}) and generator loss (\cite{ctgan}). %TableGAN adopts this idea and uses it in tabular data generation.
The information loss penalizes the discrepancy between statistics of the generated data and the real data. This helps to generate data which is statistically closer to the real one.
The classification loss requires to add to the GAN architecture an auxiliary classifier in parallel to the discriminator. 
For each synthesized label the classifier outputs a predicted label.
The classification loss quantifies the discrepancy between the synthesized and predicted class. This helps to increase the semantic integrity of synthetic records.
For instance, (sex=female, disease=prostate cancer) is not a semantically correct record as women do not have a prostate, and no such record should appear in the original data and is hence not learnt by the classifier.
%To counter this problem we incorporate an additional loss (i.e., generator loss) measuring
The generator loss measures the difference between the given conditions and the output classes of the generator. This loss helps the generator to learn to produce the exact same classes as the given conditions.
Classification loss is used by TableGAN but not CTGAN, since CTGAN does not contain classifier. Generator loss is implemented by CTGAN but not TableGAN, because TableGAN is not a conditional GAN.
% \zz{Different from the general generator loss for GANs which is back-propagated from the discriminator, our generator loss measures the difference between the given conditions and the output classes of the generator. This loss helps the generator to learn to produce the exact same classes as the given conditions.}\rb{Not clear: does this mean we ignore the feedback from discriminator? If so how does the minimax game work here? Or we add it? Maybe we can add the (high level formula) in sec 3.2?}
%is used to enforce the conditional generator. When a conditional vector is given for generator, the output of generator may not in line with the given conditional vector. Therefore, by adding cross-entropy between given conditional vector and generated classes, generator will learn to produce exact the same classes as the given conditional vector.} 

To counter complex distributions in continuous \columns we embrace the \textit{mode-specific normalization (MSN)} idea~
 (\cite{ctgan}) which encodes each value as a value-mode pair stemming from Gaussian mixture model.

% Classifier in GAN can increase the \textbf{semantic integrity} of synthetic records. For instance, (sex=man, disease=uterine cancer) is not a semantically correct record as man does not have uterine, and there should not contain such record in the original table. A classifier can help to suppress the generation of such records. But unfortunately, TableGAN does not take the imbalanced categorical column problem into consideration.

% In our design, we adopt the above-mentioned good qualities, and develop our own contributions to further improve them.

\subsubsection{Differential Privacy}

% \subsection{Training with Differential Privacy Guarantees}
% \label{ssec:dp-sgd}

% DP-SGD~\cite{abadi2016deep} is the central framework to provide DP guarantees in this work. DP-SGD uses noisy stochastic gradient descent to limit the influence of individual training samples $x_i$. After computing the gradient $g(x_i)$, the gradient is clipped based on a clipping parameter $C$ and its L2 norm  $\bar{g}(x_i) \leftarrow g(x_i)/\max(1,\frac{||g(x_i)||_{2}}{C})$, and Gaussian noise is added $\Tilde{g}(x_i)\leftarrow \bar{g}(x_i)+\mathcal{N}(0,\sigma^{2}C^{2}I))$. $\Tilde{g}$ is then used in place of $g$ to update the network parameters as in traditional SGD where $\Tilde{g}$ now fits the definition of a Gaussian mechanism $\mathcal{M}_{\sigma}$.  

% One of the biggest challenges with DP-SGD is tuning the clipping parameter $C$ since clipping greatly degrades the information stored in the original gradients~\cite{chen2020gs}. Choosing an optimal clipping value that does not significantly impact utility is crucial. However, tuning the clipping parameter is laborious as the optimal value fluctuates depending on network hyperparameters (i.e. model architecture, learning rate)~\cite{abadi2016deep}.
% To avoid an intensive hyper-parameter search, \cite{chen2020gs}~proposes to use the Wasserstein loss with a gradient penalty term.  
% This term ensures that the discriminator generates bounded gradient norms which are close to 1 under real and generated distributions. Therefore, an optimal clipping threshold of $C=1$ is obtained analytically.

\zz{DP is becoming the standard solution in privacy protection and has even been adopted by the US census department to bolster privacy of citizens~\cite{Hawes2020Implementing}. DP protects against privacy attacks by  minimizing the influence of any individual data under a privacy budget. We leverage the R\'enyi Differential Privacy (RDP)~\cite{mironov2017renyi} as it provides stricter bounds on the privacy budget. A randomized mechanism \( \mathcal{M} \) is $(\lambda,\epsilon)$-RDP with order $\lambda$, if {\small
$D_{\lambda}(\mathcal{M}(S)||\mathcal{M}(S')) = \frac{1}{\lambda-1}log\mathbb{E}_{x\sim\mathcal{M}(S)} \left[  \left(\frac{P[\mathcal{M}(S)=x]}{P[\mathcal{M}(S')=x]} \right) \right]^{\lambda-1}\leq\epsilon$
holds for any adjacent datasets $S$ and $S'$, where {\small
$D_\lambda(P||Q)=\frac{1}{\lambda-1}log\mathbb{E}_{x\sim Q}[(P(x)/Q(x))^\lambda]$}} represents the R\'enyi divergence. In addition, a $(\lambda,\epsilon)$-RDP mechanism \( \mathcal{M} \) can be expressed as:}
\color{blue}
\begin{equation}
    \label{eq:rdp-to-dp}
    (\epsilon+\frac{log1/\delta}{\lambda-1},\delta)\text{-DP}.
\end{equation}
For the purposes of this work $\mathcal{M}$ corresponds to a tabular GAN model with privacy budget $(\lambda, \epsilon)$.

RDP is a strictly stronger privacy definition than DP as it provides tighter bounds for tracking the cumulative privacy loss over a sequence of mechanisms via the Composition theorem~\cite{mironov2017renyi}. Let $\circ$ denote the composition operator. For \( \mathcal{M}_{1} \),...,\( \mathcal{M}_{k} \) all $(\lambda,\epsilon_i)$-RDP, the composition \( \mathcal{M}_{1} \)$\circ ... \circ$\( \mathcal{M}_{k} \) is
\begin{equation}
    \label{eq:composition}
    (\lambda,\sum_{i}\epsilon_{i})\text{-RDP}
\end{equation}

\cite{dwork2014algorithmic} defines a Gaussian Mechanism \( \mathcal{M}_{\sigma} \) parameterized by $\sigma$ as:
\begin{equation}
    \label{eq:gaussian_mechanism}
    \mathcal{M}_{\sigma}(x) = f(x) + \mathcal{N}(0,\sigma^{2}I)
\end{equation}
where $f$ denotes an arbitrary function with sensitivity $\Delta_{2f} = \max_{S,S'}||f(S) - f(S')||_{2}$ over all adjacent datasets $S$ and $S'$, and  $\mathcal{N}$ a Gaussian noise with zero mean and covariance $\sigma^{2}I$.
$\mathcal{M}_{\sigma}$ is $(\lambda,\frac{\lambda\Delta_{2f}^{2}}{2\sigma^{2}})$-RDP~\cite{mironov2017renyi}. 

Two more theorems are key to this work. The post processing theorem~\cite{dwork2014algorithmic} states that if \( \mathcal{M} \) satisfies $(\epsilon,\delta)$-DP, $F\circ\mathcal{M}$ will satisfy $(\epsilon,\delta)\text{-DP}$, where $F$ can be any arbitrary randomized function. Hence, it suffices to train one of the two networks in the GAN architecture with DP guarantees to ensure that the overall GAN is compatible with differential privacy.

Lastly, RDP for subsampled mechanisms~\cite{wang2019subsampled} computes the reduction in privacy cost when sub-sampling private data. Formally, let $\mathcal{X}$ be a dataset with $n$ data points and \textbf{subsample} return $m \leq n$ subsamples without replacement from $\mathcal{X}$ (subsampling rate $\gamma = m/n$).
For all integers $\lambda \geq 2 $, if a randomized mechanism $\mathcal{M}$ is $(\lambda,\epsilon(\lambda))$-RDP, then $\mathcal{M}\circ\textbf{subsample}$ is
\begin{equation}
    \label{eq:subsampling}
    (\lambda,\epsilon'(\lambda))\text{-RDP}
\end{equation}

where {\small $\epsilon'(\lambda) \leq \frac{1}{\lambda-1}log(1 + \gamma^{2}\binom{\lambda}{2}\min\left\{4(e^{\epsilon(2)}-1),e^{\epsilon(2)}\min\{2,(e^{\epsilon(\infty)}-1)^{2}\}\right\} \allowbreak$ + \\$\sum_{j=3}^{\lambda}\gamma^{j} \binom{\lambda}{j}e^{(j-1)\epsilon(j)}\min\{2,(e^{\epsilon(\infty)-1)^{j})}\})$}
\color{black}
\subsection{Design of \algo}
\label{sec:design_algorithm}
The structure of \algo comprises three blocks: Generator $\mathcal{G}$, Discriminator $\mathcal{D}$ and an auxiliary Classifier $\mathcal{C}$ (see Fig.~\ref{fig:STD}). 
Since our algorithm is based on conditional GAN, the generator requires a noise vector plus a conditional vector. Details on the conditional vector are given in Sec.~\ref{sec:condvec}. To simplify the figure, we omit the encoding and decoding of the synthetic and real data detailed in Sec.~\ref{ssec:data_representation}.

GANs are trained via a zero-sum minimax game where the discriminator tries to maximize the objective, while the generator tries to minimize it. The game can be seen as a mentor ($\mathcal{D}$) providing feedback to a student ($\mathcal{G}$) on the quality of his work. %\algo adopts the WGAN loss with gradient penalty (\cite{wgan_gp}) which is also used in CTGAN.
Here, we introduce additional feedback for $\mathcal{G}$ based on the information loss, classification loss and generator loss. The information loss matches the first-order (i.e., mean) and second-order (i.e., standard deviation) statistics of synthesized and real records. This leads the synthetic records to have the same statistical characteristics as the real records.
% In addition, the classifier is trained to learn the correlation between classes and the other \column values using the real training data.
% The classification loss helps to check the semantic integrity, and penalizes synthesized records where the combination of values are semantically incorrect.
The classification loss equates the correlation between classes and the other \column values. %using the real training data.
This helps to check the semantic integrity, and penalizes synthesized records where the combination of values are semantically incorrect.
Finally, the generator loss is the cross-entropy between the given conditional vector and the generated output classes. It enforces the conditional generator to produce the same classes as the given conditional vector.
These three losses are added to the original loss term of $\mathcal{G}$ during training.
% % To train the conditional GAN we enhance the  zero-sum minimax loss  betweenwith two extra Generator loss terms information loss and   
% Loss function is important to train the GAN. In our \algo,  we introduce the \textit{Information Loss} from table-GAN. \textit{Information Loss} matches the first-order (i.e., mean) and second-order (i.e., standard deviation) statistics of record features; thus, together with loss from Discriminator, they will lead the synthetic records to have the same statistical characteristics as the original records. The loss from Classifier helps to check the semantic integrity, and penalize the generation where the combination of values are semantically incorrect.
% The training process for one epoch within \algo is:
% \begin{itemize}
%     \item Generator $\mathcal{G}$ generates $N$ rows of synthetic data $\mathcal{T}_S$ using conditional vector $\mathcal{V}$ plus noise vector.
%   \item User samples $N$ rows of real data $\mathcal{T}_{R}$.  $\mathcal{V}$ is used during this process to make sure that each row in  $\mathcal{V}$ has a corresponding record from $\mathcal{T}_{R}$ (Details in Sec.~\ref{sec:condvec}).
%     \item $\mathcal{T}_S$ and $\mathcal{T}_R$ will individually attached with $\mathcal{V}$, and feed to Discriminator $\mathcal{D}$. We calculate the loss $\mathcal{L}_D^{\mathcal{T}_S}$ and loss  $\mathcal{L}_D^{\mathcal{T}_R}$ to train $\mathcal{D}$. Information loss $\mathcal{L}_{in}$ is also calculate between $\mathcal{T}_S$ and $\mathcal{T}_R$. Information loss and $\mathcal{L}_D^{\mathcal{T}_R}$ will return to $\mathcal{G}$.
%     \item $\mathcal{T}_S$ and $\mathcal{T}_R$ need to select out one target column from the data, and the rest columns as the inputs to the Classifier $\mathcal{C}$. %$\mbox{LossC}_{RD}$ 
%     $\mathcal{L}^{\mathcal{T}_R}_{C}$ will be used to train $\mathcal{C}$, $\mathcal{L}_C^{\mathcal{T}_R}$ will return to $\mathcal{G}$.
%     \item $\mathcal{L}_{in}$, $\mathcal{L}_D^{\mathcal{T}_R}$ and $\mathcal{L}_C^{\mathcal{T}_R}$ are used to train $\mathcal{G}$.
% \end{itemize}
%$\mathcal{G}$ and $\mathcal{D}$ are implemented by a four and a two layers CNN , respectively.
$\mathcal{G}$ and $\mathcal{D}$ are implemented using CNNs with the same structure as in~\cite{tablegan}.
% \ak{$\mathcal{G}$ consists of stacks of strided 2D convolutional transpose layers followed by a 2d batch norm layer and a relu activation function. And $\mathcal{D}$ is composed of stacks of 2d convolutional layers, 2d batch norm and LeakyReLU layers with the final output being passed through a Sigmoid activation function.} 
%\zz{@Adytia, could you add one phrase to introduce the CNN?}
CNNs are good at capturing the relation between pixels within an image, which in our case, can help to increase the semantic integrity of synthetic data. To process row records stored as vectors with CNN, we wrap the row data into the closest square matrix dimensions, i.e. $d \times d$ where $d$ is the ceiled square root of the row data dimensionality and pad missing values with zeros.
% We append the insufficient ``pixels'' in the end with 0.
% To input a row record into CNN, we need to wrap the data into a square ``image'' format.
% But instead of using a CNN for classifier in TableGAN, we use a MLP for it.
%\ak{$\mathcal{C}$ consists of 4 linear layers with 256 nodes each which are all followed by a leaky relu activation and are trained with dropout regularization with a probability parameter of 0.5. Note that the last layer of the classifier is adapted to deal with binary as well as multi-class classification problems where the sigmoid with binary cross entropy and cross entropy losses are used, respectively.}     
%\zz{@Adytia, maybe information for nodes in each layer?}
$\mathcal{C}$ uses a multi-layer-perceptron (MLP) with four 256-neuron hidden layers. The classifier is trained on the original data to better interpret the semantic integrity. Hence synthetic data are reverse transformed from their matrix encoding to vector (details in Sec.~\ref{ssec:data_representation}). Real data is encoded (details in Sec.~\ref{ssec:data_representation} and \ref{ssec:longgtail}) before being used as input for $\mathcal{C}$ to create the class label predictions.

% The original GAN \cite{gan} formulation  expressed below: 
% \begin{equation}
% \min_{\mathcal{G}}\max_{\mathcal{D}}V(\mathcal{G},\mathcal{D}) = \mathbb{E}[log\mathcal{D}(x)]_{x\sim p_{data}(x)} + \mathbb{E}[log(1-\mathcal{D}(\mathcal{G}(z)))]_{z \sim p(z)}
% \end{equation}
% where $p(z)$ denotes a prior distribution (i.e $\mathcal{N}(0,I)$) with latent vector $z$ and $\mathcal{D}$ outputs a scalar in the range [0,1], provides

% Let $\mathcal{L}^{D}_{orig}$ and $\mathcal{L}^{G}_{orig}$ denote the original GAN loss functions from~\cite{gan} to train $\mathcal{D}$ and $\mathcal{G}$, respectively.
% Let $f_x$ and $f_{\mathcal{G}(z)}$ denote the resulting features obtained from the penultimate layer of $\mathcal{D}$ for a real and generated sample, respectively.  Thus, the \textbf{information loss} for $\mathcal{G}$ is expressed as:
% $\mathcal{L}_{info}^{G}= \mathcal{L}_{mean} + \mathcal{L}_{sd}$ where $\mathcal{L}_{mean} = ||\mathbb{E}[f_x]_{x \sim p_{data}(x)} - \mathbb{E}[f_{\mathcal{G}(z)}]_{z \sim p(z)}||_{2}$ and $\mathcal{L}_{sd} = ||\mathbb{SD}[f_x]_{x \sim p_{data}(x)} - \mathbb{SD}[f_{\mathcal{G}(z)}]_{z \sim p(z)}||_{2}$. And, $\mathbb{E}$ and $\mathbb{SD}$ denote the mean and standard deviations of the features, respectively; 
% To calculate \textbf{classifier loss}. $\mathcal{L}_{class}^{C} = \mathbb{E}[|l(x)-\mathcal{C}(fe(x))|]_{x \sim p_{data}(x)}$
% $\&$
% $\mathcal{L}_{class}^{G} = \mathbb{E}[|l(G(z))-\mathcal{C}(fe(G(z)))|]_{z \sim p(z)}$ correspond to training $\mathcal{C}$ and $\mathcal{G}$, respectively, where $l(.)$ is a function that returns the class label of any given data row and $fe(.)$ deletes the class feature of that data row; 
% Let $m_{i*}$ represent the conditional masking for the selected one-hot-encoded column $i$ associated with the conditional vector $\mathcal{V}$ (refer to section \ref{sec:condvec}) for a given data row and $\hat{d}_{i*}$ denote the corresponding generated masking. The \textbf{generator loss} denoted as $\mathcal{L}_{generator}^{G}$ is formally represented as: $-\sum_{k=1}^{n}t_{j}log(p_{j})$ where n is the total number of categories in $i$, $t_j=\argmax(m_{i*})$ and $p_{j}$ is the softmax probability for the $j^{th}$ category in $i$. 

% Thus, the training objectives of the discriminator and classifier is simply given by $\mathcal{L}^{D}_{orig}$ and $\mathcal{L}_{class}^{C}$, respectively. Whereas, for the generator, the combined training objective is expressed as $\mathcal{L}^{G}=\mathcal{L}^{G}_{orig}+\mathcal{L}_{info}^{G}+\mathcal{L}_{class}^{G} + \mathcal{L}_{generator}^{G}$.

Let $f_x$ and $f_{\mathcal{G}(z)}$ denote the features fed into the softmax layer of $\mathcal{D}$ for a real sample $x$ and a sample generated from latent value $z$, respectively. The \textbf{information loss} for $\mathcal{G}$ is expressed as
$\mathcal{L}_{info}^{G} = ||\mathbb{E}[f_x]_{x \sim p_{data}(x)} - \mathbb{E}[f_{\mathcal{G}(z)}]_{z \sim p(z)}||_{2} + ||\mathbb{SD}[f_x]_{x \sim p_{data}(x)} - \mathbb{SD}[f_{\mathcal{G}(z)}]_{z \sim p(z)}||_{2}$ where $p_{data}(x)$ and $p(z)$ denote prior distributions for real data and latent variable, $\mathbb{E}$ and $\mathbb{SD}$ denote the mean and standard deviations of the features, respectively. %\lc{Lets stress classifier loss is new on top of CTGAN.}
The \textbf{classifier loss} is given by 
% $\mathcal{L}_{class}^{C} = \mathbb{E}[|l(x)-\mathcal{C}(fe(x))|]_{x \sim p_{data}(x)}$
% and 
$\mathcal{L}_{class}^{G} = \mathbb{E}[|l(G(z))-\mathcal{C}(fe(G(z)))|]_{z \sim p(z)}$
% correspond to training $\mathcal{C}$ and $\mathcal{G}$, respectively,
where $l(.)$ returns the target label and $fe(.)$  returns the input features of a given row $x$.
Finally, the \textbf{generator loss} is given by  $\mathcal{L}_{generator}^{G} = H(m_{i}, \hat{m}_{i})$ where $m_{i}$ and $\hat{m}_i$ are the given and generated conditional vector bits corresponding to column $i$ and $H(.)$ is the cross-entropy loss. Columns are selected using the training-by-sampling procedure (see Sec.~\ref{sec:condvec} for details).


% Let $m_{i*}$ represent the conditional masking for the selected one-hot-encoded column $i$ associated with the conditional vector $\mathcal{V}$ (refer to section \ref{sec:condvec}) for a given data row and $\hat{d}_{i*}$ denote the corresponding generated masking. The \textbf{generator loss} denoted as $\mathcal{L}_{generator}^{G}$ is formally represented as: $-\sum_{k=1}^{n}t_{j}log(p_{j})$ where n is the total number of categories in $i$, $t_j=\argmax(m_{i*})$ and $p_{j}$ is the softmax probability for the $j^{th}$ category in $i$. 

Let $\mathcal{L}^{D}_{orig}$ and $\mathcal{L}^{G}_{orig}$ denote the original GAN loss functions from~\cite{gan} to train the discriminator $\mathcal{D}$ and generator $\mathcal{G}$, respectively. For $\mathcal{G}$ the complete training objective is the combination of $\mathcal{L}^{G}=\mathcal{L}^{G}_{orig}+\mathcal{L}_{info}^{G}+\mathcal{L}_{class}^{G} + \mathcal{L}_{generator}^{G}$, while for $\mathcal{D}$ it is unchanged, i.e. $\mathcal{L}^{D}_{orig}$. Finally, the loss to train the classifier  $\mathcal{C}$ is similar to the classification loss of the generator, i.e. $\mathcal{L}_{class}^{C} = \mathbb{E}[|l(x)-\mathcal{C}(fe(x))|]_{x \sim p_{data}(x)}$.


% \ak{The loss functions for CTABGAN are as follows:

% \begin{enumerate}

% \item The original GAN \cite{gan} formulation  expressed below : 
% \begin{equation}
% \min_{\mathcal{G}}\max_{\mathcal{D}}V(\mathcal{G},\mathcal{D}) = \mathbb{E}[log\mathcal{D}(x)]_{x\sim p_{data}(x)} + \mathbb{E}[log(1-\mathcal{D}(\mathcal{G}(z)))]_{z \sim p(z)}
% \end{equation}

% where $p(z)$ denotes a prior distribution (i.e $\mathcal{N}(0,I)$) with latent vector $z$ and $\mathcal{D}$ outputs a scalar in the range [0,1], provides $\mathcal{L}^{D}_{orig}$ $\&$ $\mathcal{L}^{G}_{orig}$ denoting the original loss functions for training $\mathcal{D}$ $\&$ $\mathcal{G}$, respectively. 

% \item Information Loss \cite{tablegan}: Let $f_x$ $\&$ $f_{\mathcal{G}(z)}$ denote the resulting features obtained from the penultimate layer of $\mathcal{D}$ for a real and generated sample, respectively.  Thus, the information loss for $\mathcal{G}$ is expressed as:
% $\mathcal{L}_{info}^{G}= \mathcal{L}_{mean} + \mathcal{L}_{sd}$ where $\mathcal{L}_{mean} = ||\mathbb{E}[f_x]_{x \sim p_{data}(x)} - \mathbb{E}[f_{\mathcal{G}(z)}]_{z \sim p(z)}||_{2}$ and $\mathcal{L}_{sd} = ||\mathbb{SD}[f_x]_{x \sim p_{data}(x)} - \mathbb{SD}[f_{\mathcal{G}(z)}]_{z \sim p(z)}||_{2}$. And, $\mathbb{E}$ and $\mathbb{SD}$ denote the mean and standard deviations of the features, respectively. 


% \item Classifier Loss \cite{tablegan}: $\mathcal{L}_{class}^{C} = \mathbb{E}[|l(x)-\mathcal{C}(remove(x))|]_{x \sim p_{data}(x)}$
% $\&$
% $\mathcal{L}_{class}^{G} = \mathbb{E}[|l(G(z))-\mathcal{C}(remove(G(z)))|]_{z \sim p(z)}$ correspond to training $\mathcal{C}$ and $\mathcal{G}$, respectively, where $l(.)$ is a function that returns the class of any given data row and $remove(.)$ deletes the class feature of that data row. 

% \item Generator Loss \cite{ctgan}: Let $m_{i*}$ represent the conditional masking for the selected one-hot-encoded column $i$ associated with the conditional vector $\mathcal{V}$ (refer to section \ref{sec:condvec}) for a given data row and $\hat{d}_{i*}$ denote the corresponding generated masking. The generator loss denoted as $\mathcal{L}_{generator}^{G}$ is formally represented as: $-\sum_{k=1}^{n}t_{j}log(p_{j})$ where n is the total number of categories in $i$, $t_j=\argmax(m_{i*})$ and $p_{j}$ is the softmax probability for the $j^{th}$ category in $i$. 
% \end{enumerate} 


% Thus, the training objectives of the discriminator and classifier is simply given by $\mathcal{L}^{D}_{orig}$ and $\mathcal{L}_{class}^{C}$, respectively. Whereas, for the generator, the combined training objective is expressed as $\mathcal{L}^{G}=\mathcal{L}^{G}_{orig}+\mathcal{L}_{info}^{G}+\mathcal{L}_{class}^{G} + \mathcal{L}_{generator}^{G}$.
% }








%\ak{With respect to the above sentence about trianing classifier with original data. We actually train the classifier using the BGM encoded format of the data. It's not reverse transformed before feeding into the classifier.}

%\ak{I want to also discuss about the following: After the encoding described in section 3.3 is performed, we take inspiration from \cite{tablegan} and encode this transformed tabular data into an image format by converting each row into a square matrix and pad with zeros if necessary to do so. For example, if we have rows of 8 columns each, we pad with an additional column with zero values to then convert each row into a square matrix of dimension 3x3. I want to also try to see if we can use rectangular convolutions but this is maybe an experiment for future investigations. In any case, moving on. This square form of the data is then used by the $\mathcal{G}$ and $\mathcal{D}$ described previously. Note that the output of the generator is reshaped to a tabular format and the padded values are removed for applying the final activation function. For numeric columns a tanh activation function is used and for the one-hot-encoded categorical columns, the gumbel-softmax activation function is used. Finally, the conditional vector is appended to the generated reshaped tabular data and converted back into a square form as mentioned previously to be used as input for the discriminator whereas for the classifier module, the tabular format is used as is. }

% \ak{added subsection for the general transformer}
\subsection{General Transform} \ak{The general transform is an effective approach to minimize the complexity of our algorithm. It is a simple reversible transformation than can be applied to both continuous and categorical columns before feeding them into the model.}

\ak{In the case of continuous columns, each data point is first normalized to lie between 0 and 1 and subsequently scaled to lie between the range of $(-1,1)$ so as to be compatible with a tan-h activation function. Mathematically, this can be described as follows, given a data point $x_i$ belonging to a numerical column $x$ in the original dataset, the transformed value, $g_{x_i} = 2*\frac{x_i - min(x)}{max(x)-min(x)} - 1$ where $min(x)$ and $max(x)$ represents the minimum and maximum values of the respective numeric column. Likewise a corresponding generated value $t_i$ belonging to column x may be reverse transformed as $g_{t_i}=(max(x)-min(x))*\frac{t_i+1}{2}+min(x)$.}

\ak{In the case of categorical columns, each category is encoded with a numeric integer which is then treated in a similar fashion as numeric columns with the only difference being that inverse transformed values are rounded back to numeric integers to correspond to any given category.}

\ak{The main use-case of this transformation in the context of numeric columns is to effectively reduce the computational burden needed for processing numeric columns via the mode-specific normalisation. This not only reduces the dimensionality of the data fed to the model but is also especially beneficial in specific scenarios where certain numeric distributions can be described simply using a single mode. The figures~\ref{fig:wgmm} and~\ref{fig:wogmm} shown below illustrate this phenomenon in detail and show how using the general transform can help produce more realistic column distributions for simple and smooth looking single-mode gaussian distributions such as the "Age" column in the Adult dataset.}

\begin{figure}[t]
	\begin{center}
		\subfloat[Age \column distribution with VGM]{
			\includegraphics[width=0.47\columnwidth]{figures/With GMM.jpg}
			\label{fig:wgmm}
		}
		\hfil
		\subfloat[Age \column distribution without VGM]{
			\includegraphics[width=0.47\columnwidth]{figures/Without GMM.jpg}
			\label{fig:wogmm}
		}
		\caption{VGM vs General transform of Age \column in Adult dataset}
		\label{fig:gmm_distribution}
	\end{center}
% 	\vspace{-0.5em}
\end{figure}

\ak{Similarly, in the context of categorical columns, the general transform serves as an effective means to generate high-dimensional categorical variables more easily while saving on the huge blow-up in input dimensionality caused by utilizing a one-hot-encoding representation. This serves to reduce both the time and space complexity of the algorithm significantly and boosts performance especially for small datasets such as the loan dataset where conditional training on a high-dimensional input dataset can lead to difficulties in the training efficiency and cause poor convergence. }

% Will refer to experimental evidence showcasing improvement on loan dataset in both time efficiency and generated data quality 

\ak{However, a major caveat of this approach is that due to the elimination of the mode-specific-normalisation for numeric columns and one-hot-encoding of categorical columns, the model is no longer conditionally trained with respect to these transformed columns and this can lead to negative consequences when there are important correlations that must be learnt between these columns with rest of the data. Additionally, one must rely on user-expertise to carefully select the columns which must be transformed and conduct extensive experiments to validate it's efficacy in practical real-world use-cases. Finally, the approach of rounding for processing categorical columns as if they are numerical distributions is not theoretically well justified.}

\subsection{\encoder}
\label{ssec:data_representation}

% \begin{figure}[t]
% 	\begin{center}
% 		\subfigure[\footnotesize{Mixed type \column distribution with VGM}]{
% 			\includegraphics[width=0.3\columnwidth]{figures/bi-mode-4.png}
% 			\label{fig:vgm}
% 		}
% 		\hfil
% 		\subfigure[\footnotesize{Mode selection of single value in continuous \column}]{
% 			\includegraphics[width=0.3\columnwidth]{figures/bi-mode-7.png}
% 			\label{fig:vgm_single}
% 		}
% 		\caption{Encoding for mix data type \column}
% 		\label{fig:gmm_distribution}
% 	\end{center}
% 	\vspace{-1.5em}
% \end{figure}


\begin{figure}[t]
	\begin{center}
		\subfloat[Mixed type \column distribution with VGM]{
			\includegraphics[width=0.47\columnwidth]{figures/bi-mode-4.png}
			\label{fig:vgm}
		}
		\hfil
		\subfloat[Mode selection of single value in continuous \column]{
			\includegraphics[width=0.47\columnwidth]{figures/bi-mode-7.png}
			\label{fig:vgm_single}
		}
		\caption{Encoding for mix data type \column}
		\label{fig:gmm_distribution}
	\end{center}
% 	\vspace{-0.5em}
\end{figure}


% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.50\textwidth}
% 	\begin{center}
% 		\subfigure[\footnotesize{Mixed type}]{
% 			\includegraphics[width=0.45\columnwidth]{figures/bi-mode-4.png}
% 			\label{fig:vgm}
% 		}
% 		\hfil
% 		\subfigure[\footnotesize{Mode selection}]{
% 			\includegraphics[width=0.42\columnwidth]{figures/bi-mode-7.png}
% 			\label{fig:vgm_single}
% 		}
% 		\vspace{-0.5em}
% 		\caption{Encoding for mix data type \column}
% 		\label{fig:gmm_distribution}
% 	\end{center}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.44\textwidth}
%     \centering
%     \includegraphics[width=0.9\columnwidth]{figures/condvec_1.png}
%      \vspace{-0.5em}
%     \caption{Conditional vector $\mathcal{V}$ example}
%     %\vspace{-0.5em}
%     \label{fig:condvec}
%   \end{minipage}
%   \vspace{-2em}
% \end{figure}


The tabular data is encoded \column by \column. We distinguish three types of \columns: categorical, continuous and \mixed. 
%\zz{Before introducing the data types, one thing to be notice is that we assume that the user already knows the data type of each variable before training. \cite{ctgan} holds the same assumptions.}
% \textbf{\encoder}.
We define \columns as mixed if they contain both categorical and continuous values or continuous values with missing values. We propose the new \encoder to deal with such \columns. With this encoder, values of \mixed \columns are seen as concatenated value-mode pairs. We illustrate the encoding via the exemplary distribution of a \mixed \column shown in red in Fig.~\ref{fig:gmm_distribution}(a). One can see that values can either be exactly $\mu_0$ or $\mu_3$ (the categorical part) or distributed around two peaks in $\mu_1$ and $\mu_2$ (the continuous part). We treat the continuous part using a variational Gaussian mixture model (VGM) (\cite{prml}) to estimate the number of modes $k$, e.g. $k=2$ in our example, and fit a Gaussian mixture. The learned Gaussian mixture is $\mathbb{P} = \sum_{k=1}^{2} \omega_k \mathcal{N}(\mu_k, \sigma_k)$, 
where $\mathcal{N}$ is the normal distribution and $\omega_k$, $\mu_k$ and $\sigma_k$ are the weight, mean and standard deviation of each mode, respectively.

To encode values in the continuous region of the \column distribution, we associate and normalize each value with the mode having the highest probability (see Fig.~\ref{fig:gmm_distribution}(b)). Given $\rho_1$ and $\rho_2$ being the probability density from the two modes in correspondence of the \column value $\tau$ to encode, we select the mode with the highest probability. In our example $\rho_1$ is higher and we use mode $1$ to normalize $\tau$. The normalized value $\alpha$ is: $\alpha =  \frac{\tau - \mu_1}{4\sigma_1}$.
Moreover we keep track of the mode $\beta$ used to encode $\tau$ via one-hot encoding, e.g.  $\beta = [0,1,0,0]$ in our example. The final encoding is giving by the concatenation of $\alpha$ and $\beta$: $\alpha \bigoplus \beta$
\ifshowntationtable
.
\else
where $\bigoplus$ is the vector concatenation operator.
\fi
The categorical part (e.g., $\mu_0$ or $\mu_3$ in Fig.~\ref{fig:gmm_distribution}(a)) is treated similarly, except $\alpha$ is directly set to 0. Because the category is determined only by one-hot encoding part. For example, for a value in $\mu_3$, the final encoding is given by $0 \bigoplus [0, 0, 0, 1]$.
% The categorical values are treated similarly, except $\alpha$ directly represents the value of the mode, e.g. corresponding to $\mu_0$ or $\mu_3$ in our example. Hence, for a value in $\mu_3$, the final encoding is given by $0 \bigoplus [0, 0, 0, 1]$. Note that categorical values are not limited to numbers. They can be of any type such as a string or even missing. We can map these symbols to a numeric value outside of the range of the continuous region.
Categorical \columns use the same encoding as the continuous intervals of \mixed \columns. 
Categorical \columns are encoded via a one-hot vector $\gamma$. Missing values are treated as a separate unique class and we add an extra bit to the one-hot vector for it. A row with $[1, \dots, N]$ \columns is encoded by concatenation of the encoding of all \column values, i.e. either $(\alpha \bigoplus \beta)$ for continuous and mixed \columns or $\gamma$ for categorical \columns. %, sorted by column type.
Having $n$ continuous/mixed \columns and $m$ categorical \columns ($n + m = N$) the final encoding is: %\rb{zilong check this. Also why is he ordering important?}:    
%\vspace{-0.5em}
\begin{equation}
\label{condvec}
    \bigoplus_{i=1}^{n} \alpha_i\mathsmaller{\bigoplus} \beta_{i} \;
    \bigoplus_{j=n+1}^{N} \gamma_{j} 
\end{equation}

%%%% Alternative: to be fixed if used
% \begin{equation}
% \label{condvec}
%     (\alpha_1\mathsmaller{\bigoplus} \beta_{1}) \; \bigoplus
%     \dots (\alpha_2\mathsmaller{\bigoplus} \beta_{2})
%      \; \bigoplus
%     \dots
%      \gamma_{N-1} \; \bigoplus
%     \;\gamma_{N}
% \end{equation}

% In the end, if we want to encode a pure continuous column without missing value, we can simply use only the encoding for continuous part from mix-type encoder. Therefore, for representing one row $i$ in a tabular data using our encoder, the row transferred as: 
% \begin{equation}
% \label{condvec}
%     \alpha_{i,N_w}\mathsmaller{\bigoplus} \beta_{i,N_w}\mathsmaller{\bigoplus} \cdot\cdot\cdot \mathsmaller{\bigoplus} \alpha_{i,N_x}\mathsmaller{\bigoplus} \beta_{i,N_x}\mathsmaller{\bigoplus}\gamma_{i,N_y}\mathsmaller{\bigoplus} \cdot\cdot\cdot  \mathsmaller{\bigoplus} \gamma_{i,N_z} 
% \end{equation}
% where $\gamma_{i,j}$ represents the one-hot encoding vector for $i$th row value in categorical column $j$.


% If the column is defined as categorical column, one-hot encoding will be used to transfer the values. Missing value in categorical column will be seen as an unique class, we will add one bit in the one-hot vector for it.


% For continuous columns, we partially adapt the \textit{Mode-specific Normalization} idea from~\cite{ctgan} in using variational Gaussian mixture model (VGM)~\cite{prml} to estimate the number of modes and fit a Gaussian mixture. To represent mixed data type and missing value in column containing continuous values, a new data type \bimodal is defined for that. And a new method \textbf{Mix-Type Encoder} is proposed to deal with that type of column. %We will show that Mix-Type Encoder can deal with the case where a column only contains continuous value or mix data type, whether it contains missing value or not.


% \textbf{Encode for continuous part}: For example, for a mix data type column $C_j$ in tabular data \mbox{TD}, the distribution is shown as the red curves in Fig.~\ref{fig:vgm}. We can see that there are two single mode $\mu_0$ and $\mu_3$, they are actually categorical values. And in the middle place, it is obviously a continuous distribution, the VGM finds two modes namely: $\mu_1$ and $\mu_2$. $\mu_1$ and $\mu_2$ represent also the mean values for these two modes. 
%     The learned Gaussian mixture is:
% \begin{equation}
%     \mathbb{P}_{C_j} =  \sum_{k=1}^{2} \omega_k \mathcal{N}(\mu_k, \sigma_k)
% \end{equation}
% where $\omega_k$ and $\sigma_k$ are the weight and standard deviation of a mode respectively.

% As shown in the Fig.~\ref{fig:vgm_single}. For each value $\tau_{i,j}$ in column $C_{j}$, calculates the probability of $\tau_{i,j}$ coming from each mode. The $\rho_0$ and $\rho_1$ are the probability density from the two modes. And we pick the mode with higher probability density (i.e., $\rho_0$ in Fig.~\ref{fig:vgm_single}) to normalize $\tau_{i,j}$. The normalized value $\alpha_{i,j}$ of $\tau_{i,j}$ using mode $\mu_1$ is:
% \begin{equation}
%     \alpha_{i,j} =  \frac{\tau_{i,j} - \mu_1}{4\sigma_1}
% \end{equation}
% In addition to encoding the value itself, mode information also needs to be encoded, as we have four modes in column $C_{j}$, the mode information $\beta_{i,j}$ for $\tau_{i,j}$ is represented as:
% \begin{equation*}
%     \beta_{i,j} = [0,1,0,0]
% \end{equation*}
% where the 1 in $\beta_{i,j}$ indicates that we choose mode $mu_1$ to normalize $\tau_{i,j}$. Therefore, the encoding for $\tau_{i,j}$ is $\alpha_{i,j}\bigoplus \beta_{i,j}$.

% \textbf{Encode for categorical part}: After normalizing the continuous value in column $C_j$, let us check the categorical value $\mu_0$ and $\mu_1$. If a categorical value $\tau_{i,j}$ equals to $\mu_0$, then the encoded value $\alpha_{i,j}$ of $\tau_{i,j}$ is directly equals to $\mu_0$. One should notice that the categorical value is not limited to only numeric value, it can be string or even empty, we can map these symbols to a numeric value outside the range of continuous part. And for categorical part, the mode also need to be encoded. To conclude, for a value $\tau_{k,j} = \mu_0$ in column $C_j$, its encode is $\alpha_{k,j}\bigoplus \beta_{k,j} $ where:
% \begin{align*}
%     \alpha_{k,j} = \mu_0, \quad \beta_{k,j} = [1,0,0,0]
% \end{align*}

% In the end, if we want to encode a pure continuous column without missing value, we can simply use only the encoding for continuous part from mix-type encoder. Therefore, for representing one row $i$ in a tabular data using our encoder, the row transferred as: 
% \begin{equation}
% \label{condvec}
%     \alpha_{i,N_w}\mathsmaller{\bigoplus} \beta_{i,N_w}\mathsmaller{\bigoplus} \cdot\cdot\cdot \mathsmaller{\bigoplus} \alpha_{i,N_x}\mathsmaller{\bigoplus} \beta_{i,N_x}\mathsmaller{\bigoplus}\gamma_{i,N_y}\mathsmaller{\bigoplus} \cdot\cdot\cdot  \mathsmaller{\bigoplus} \gamma_{i,N_z} 
% \end{equation}
% where $\gamma_{i,j}$ represents the one-hot encoding vector for $i$th row value in categorical column $j$.

% \subsection{Conditional vector construction}
% \vspace{-0.6em}
\subsection{Counter \Imbalanced Training Datasets}
\label{sec:condvec}

In \algo, we use conditional GAN to counter imbalanced training datasets using training-by-sampling (\cite{ctgan}), but extended to include the modes of continuous and mixed columns.
When we sample real data, we use the conditional vector to filter and rebalance the training data. 
The conditional vector $\mathcal{V}$ is a bit vector given by the concatenation of all mode one-hot encodings $\beta$ (for continuous and \mixed \columns) and all class one-hot encodings $\gamma$ (for categorical \columns) for all \columns present in Eq.~\eqref{condvec}. Each conditional vector specifies a single mode or a class. More in detail, $\mathcal{V}$ is a zero vector with a single one in correspondence to the selected \column with selected mode/class.
Fig.~\ref{fig:condvec} shows an example with three \columns, one continuous ($C_1$), one \mixed ($C_2$) and one categorical ($C_3$), with class 2 selected on $C_3$. %\rb{modify figure 4 to reflect this text}. 



To rebalance the dataset, each time we need a conditional vector during training, we first randomly choose a \column with uniform probability. Then we calculate the probability distribution of each mode (or class for categorical \columns) in that \column using frequency as proxy and sample a mode based on the logarithm of its probability. Using the log probability instead of the original frequency gives minority modes/classes higher chances to appear during training. This helps to alleviate the collapse issue for rare modes/classes. Extending the conditional vector to include the continuous and \mixed \columns helps to deal with imbalance in the frequency of modes used to represent them.
Moreover, since generator is conditioned on all data-types during training,  this enhances the learned correlation between all \columns.
%Extending the conditional vector to include the continuous and \mixed \columns helps to deal with imbalance in the frequency of modes used to represent them.
%Moreover, since generator in \algo is conditioned on all data-types during training,  this enhances the learned correlation between all \columns. %(refer to statistical similarity results in Tab. \ref{table:ML_all}).}

\begin{figure}[t]
    \centering
    \includegraphics[scale=.18]{figures/condvec_1.png}
    \caption{Conditional vector: example selects class 2 from third \column out of three}
    \label{fig:condvec}
     %\vspace{-1em}
\end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=.18]{figures/condvec_1.png}
%     \vspace{-0.5em}
%     \caption{Conditional vector: example selects class 2 from third \column out of three}
%     %\vspace{-0.5em}
%     \label{fig:condvec}
%      \vspace{-1em}
% \end{figure}


% Recall the encoded row from Eq.\eqref{condvec}. All the sub-vectors $\beta$ and $\gamma$ are one-hot encoding.  To organise a conditional vector for the dataset that Eq.\eqref{condvec} resides in, we first initialize a vector of the length as the sum of length of all $\beta$ and $\gamma$ sub-vectors in Eq.\eqref{condvec}. We initialize the vector with 0 in all the bit. And every time when we need a conditional vector, we first randomly select a column $j^*$. Once we locate one column, we calculate a probability distribution of each mode (or class for categorical column) in the column by the logarithm of frequency. And we select a mode $k^*$ within this column by this probability distribution. Using logarithm instead of original frequency gives more chance for the minority mode or class to be sampled out, and can help to solve the mode collapse issue. A conditional vector can be defined as:
% \begin{equation}
% \mbox{Conditional Vector } \mathcal{V}_{j}^{k} =  \left\{
% 	\begin{array}{rl}
% 		 \mbox{1} &  \mbox{if $j$=$j^*$, $k$=$k^*$} \\
% 		\mbox{0} & \mbox{otherwise} 	 
% 	\end{array} \right.
% \end{equation}

% A conditional vector generation process for an example with two columns is illustrated in Fig.~\ref{fig:condvec}. 


% \subsection{Data pre-processing}

% \vspace{-0.5em}
\subsection{Treat Long Tails}
\label{ssec:longgtail}
We encode continuous values using variational Gaussian mixtures to treat multi-mode data distributions (details in Sec.~\ref{ssec:data_representation}).
However, Gaussian mixtures can not deal with all types of data distribution, notably distributions with long tail where few rare points are far from the bulk of the data.
VGM has difficulty to encode the values towards the tail.
To counter this issue we pre-process \columns with long tail distributions with a logarithm transformation. For such a \column having values with lower bound $l$, we replace each value $\tau$ with compressed $\tau^c$:
%\vspace{-1em}
\begin{equation}
\label{eq:preprossesing}
\tau^c =  \left\{
	\begin{array}{rl}
		 \mbox{log($\tau$)} &  \mbox{if $l>$0} \\
		\mbox{log($\tau$ - $l$+$\epsilon$)} & \mbox{if $l\leqslant$0}  \mbox{, where } \mbox{$\epsilon>$0} 	 
	\end{array} \right\}
\end{equation}

The log-transform allows to compress and reduce the distance between the tail and bulk data making it easier for VGM to encode all values, including tail ones. We show the effectiveness of this simple yet performant method in Sec.~\ref{sec:further}.
% \vspace{-0.4em}

\subsection{Differential Privacy}
\label{ssec:dp-sgd}
DP-SGD~\cite{abadi2016deep} is the central framework to provide DP guarantees in this work. DP-SGD uses noisy stochastic gradient descent to limit the influence of individual training samples $x_i$. After computing the gradient $g(x_i)$, the gradient is clipped based on a clipping parameter $C$ and its L2 norm  $\bar{g}(x_i) \leftarrow g(x_i)/\max(1,\frac{||g(x_i)||_{2}}{C})$, and Gaussian noise is added $\Tilde{g}(x_i)\leftarrow \bar{g}(x_i)+\mathcal{N}(0,\sigma^{2}C^{2}I))$. $\Tilde{g}$ is then used in place of $g$ to update the network parameters as in traditional SGD where $\Tilde{g}$ now fits the definition of a Gaussian mechanism $\mathcal{M}_{\sigma}$.  

One of the biggest challenges with DP-SGD is tuning the clipping parameter $C$ since clipping greatly degrades the information stored in the original gradients~\cite{chen2020gs}. Choosing an optimal clipping value that does not significantly impact utility is crucial. However, tuning the clipping parameter is laborious as the optimal value fluctuates depending on network hyperparameters (i.e. model architecture, learning rate)~\cite{abadi2016deep}.
To avoid an intensive hyper-parameter search, \cite{chen2020gs}~proposes to use the Wasserstein loss with a gradient penalty term.  
This term ensures that the discriminator generates bounded gradient norms which are close to 1 under real and generated distributions. Therefore, an optimal clipping threshold of $C=1$ is obtained analytically.

\algoplus trains the discriminator using differential private-SGD where the number of training iterations is determined based on the total privacy budget $(\epsilon$,$\delta)$. Thus, to compute the number of iterations, the privacy budget spent for every iteration must be bounded and accumulated. %over training iterations.
For this purpose we use the subsampled RDP analytical moments accountant technique. % (\cite{wang2019subsampled}).
The theoretical analysis of the privacy cost is presented below:

\begin{cor}
Each discriminator update satisfies $(\lambda,2B\lambda/\sigma^{2})$-RDP where $B$ is the batch size.
\end{cor}

\begin{proof}
Let $f=clip({\bar{g}_D},C)$ be the clipped gradient of the discriminator before adding noise. The sensitivity is derived via the triangle inequality:
\begin{equation}
    \Delta_{2}f = \max_{S,S'}||f(S)-f(S')||_{2} \leq 2C
\end{equation}

Since $C=1$ as a consequence of the Wasserstein loss with gradient penalty %(\cite{gulrajani2017improved})
and by using \eqref{eq:gaussian_mechanism} the DP-SGD procedure denoted as $\mathcal{M}_{\sigma,C}$ parameterized by noise scale $\sigma$ and clipping parameter $C$ may be represented as being $(\lambda,2\lambda/\sigma^{2})$-RDP. 

Furthermore, each discriminator update for a batch of real data points $\{x_i,..,x_B\}$ can be represented as 

\begin{equation}
    \Tilde{g}_D = \frac{1}{B}\sum_{i=1}^{B}\mathcal{M}_{\sigma,C}(\triangledown_{\theta_D}\mathcal{L}_{D}(\theta_D,x_i))
\end{equation}

where $\tilde{g}_{D}$ and $\theta_{D}$ represent the perturbed gradients and the weights of the discriminator network, respectively. This may be regarded as a composition of $B$ Gaussian mechanisms and treated via \eqref{eq:composition}. The privacy cost for a single gradient update step for the discriminator can be expressed as $(\lambda,\sum_{i=1}^{B}2\lambda/\sigma^{2})$ or equivalently $(\lambda,2B\lambda/\sigma^{2})$.
\end{proof}

Note that $\mathcal{M}_{\sigma,C}$ is only applied for those gradients that are computed with respect to the real training dataset~\cite{abadi2016deep,zhang2018differentially}. Hence, the gradients computed with respect to the synthetic data and the gradient penalty term are left undisturbed. Next, to further amplify the privacy protection of the discriminator, we rely on~\eqref{eq:subsampling} with subsampling rate $\gamma=B/N$ where $B$ is the batch size and $N$ is the size of the training dataset. Intuitively, subsampling adds another layer of randomness and enhances privacy by decreasing the chances of leaking information about particular individuals who are not included in any given subsample of the dataset.

Lastly, it is worth mentioning that the Wasserstein loss with gradient penalty training objective has one major pitfall with respect to the privacy cost. This is because, it encourages the use of a stronger discriminator network to provide more meaningful gradient updates to the generator. This requires performing multiple updates to the discriminator for each corresponding update to the generator leading to a faster consumption of the overall privacy budget.

==> motivation.tex <==
\subsection{Motivation}
\label{sec:motivation}
% 1. mix data type problem (here show a figure about the mortgage \column in loan data, plot it in one figure).
% 2. missing value, only state on text
% 3. 

We empirically demonstrate how the prior state-of-the-art methods fall short in solving challenges in industrial data sets. The detailed experimental setup can be found in Sec.~\ref{ssec:setup}.


\textbf{\Mixed data type \columns}. To the best of our knowledge, existing GAN-based tabular generators only consider table columns as either categorical or continuous. However, in reality, a \column can be a mix of these two types, and often \columns have missing values. 
The \textit{Mortgage} \column from the Loan dataset is a good example of \bimodal variable.
Fig.~\ref{fig:motivationcases}(a) shows the distribution of the original and synthetic data generated by 4 state-of-the-art algorithms for this \column.
According to the data description, a loan holder can either have no mortgage (0 value) or a mortgage (any positive value). In appearance this \column is not a categorical type due to the numeric nature of the data. So all 4 state-of-the-art algorithms treat this \columns as continuous type without capturing the special meaning of the value zero. Hence, all 4 algorithms generate a value around 0 instead of exact 0. And the negative values for Mortgage have no/wrong meaning in the real world. 


\textbf{Long tail distributions}. Many real world data can have long tail distributions where most of the occurrences happen near the initial value of the distribution, and rare cases towards the end.
Fig.~\ref{fig:motivationcases}(b) plots the cumulative frequency for the original (top) and synthetic (bottom) data generated by 4 state-of-the-art algorithms for the
% long tail column 
\textit{Amount} in the Credit dataset. This \column represents the transaction amount when using credit cards. One can imagine that most transactions have small amounts, ranging from few bucks to thousands of dollars. However, there definitely exists a very small number of transactions with large amounts. Note that for ease of comparison both plots use the same x-axis, but Real has no negative values. %\rb{adapt to figure}.
% scaled to the same right limit.
Real data clearly has 99\% of occurrences happening at the start of the range, but the distribution extends until around $25000$. In comparison none of the synthetic data generators is able to learn and imitate this behavior.
    
%      \begin{figure}[htb]
% 	\begin{center}
% 		\subfloat[Real]{
% 			\includegraphics[width=0.48\columnwidth]{figures/real_longtail_moti.png}
% 			\label{fig:real_gmm}
% 		}
% 		\subfloat[Comparisons]{
% 			\includegraphics[width=0.48\columnwidth]{figures/state_gmm.png}
% 			\label{fig:comparison_longtail}
% 		}
% 		\caption{Cumulative frequency for the generation for \column \textit{Amount} in Credit dataset}
% 		\label{fig:gmm_result_motivation}
% 	\end{center}
% \end{figure}

\textbf{\Skewed multi-mode continuous variables}.
%\lc{is this also called \imbalanced data? We just need to stick with one terminologies. }
The term \textit{multi-mode} is extended from Variational Gaussian Mixtures (VGM). More details are given in Sec.~\ref{ssec:data_representation}. The intuition behind using multiple modes can be easily captured from Fig.~\ref{fig:motivationcases}(c). The figure plots in each row the distribution of the working \textit{Hours-per-week} \column from the Adult dataset.
% Fig.~\ref{fig:motivationcases} plots the average working hours per week for adult, and
This is not a typical Gaussian distribution.
There is an obvious peak at 40 hours but with several other lower peaks, e.g. at 50, 20 and 45. 
% But this distribution is not a typical Gaussian distribution, we can see that at 50, there is another lower peak. And 
Also the number of people working 20 hours per week is higher than those working 10 or 30 hours per week.
This behavior is difficult to capture for the state-of-the-art data generators (see subsequent rows in Fig.\ref{fig:motivationcases}(c)). The closest results are obtained by \ctgan which uses Gaussian mixture estimation for continuous variables. However, \ctgan loses some modes compared to the original distribution.
% Even though CTGAN does not reproduce the total distribution as original, since it uses Gaussian mixture estimation for the continuous \column, it still largely outperforms other comparisons. And apparently, CTGAN loses some modes comparing to original distribution.
    
% \begin{figure}[htb]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{figures/extended_condvec_5.png}
%     \caption{Generation for continuous \column \textit{Hours-per-week} in Adult dataset}
%     \label{fig:extended_vector_motivation}
% \end{figure



The above examples show the shortcomings of current state-of-the-art GAN-based tabular data generation algorithms % . fail to recover some types of data, 
and motivate the design of our proposed \algo.


==> table1.tex <==
\begin{table}[t]
\begin{minipage}{.49\linewidth}
    \centering
    \caption{Difference in ML utility}
    % \label{tab:first_table}
    \medskip
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Accuracy} & \textbf{F1-score}  & \textbf{AUC} \\
\hline
\small{\algo}    & \textbf{8.90\%} & \textbf{0.107} &   \textbf{0.094}  \\
\small{CTGAN}    &21.51\% & 0.274 &   0.253 \\
\small{TableGAN} &11.40\%  & 0.130 &   0.169  \\
\small{MedGAN}    & 14.11\%&  0.282&   0.285 \\
\small{CW-GAN}    &  20.06\%& 0.354 &  0.299 \\
\hline
\end{tabular}
}
 \label{table:ML_all}
\end{minipage}\hfill
\begin{minipage}{.43\linewidth}
    \centering
    \caption{Statistical similarity}
    \label{tab:second_table}
    \medskip
    \resizebox{1\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Method} & \textbf{Avg JSD} & \textbf{Avg WD}  & \textbf{Diff. Corr.} \\
\hline
\small{\algo}    & \textbf{0.062}  &  \textbf{1197}  &  \textbf{2.09} \\
\small{CTGAN}    & 0.0704 &  1769  & 2.73  \\
\small{TableGAN} & 0.0796 & 2117   &  2.30 \\
\small{MedGAN}   & 0.2135 & 46257  &   5.48   \\
\small{CW-GAN}   & 0.1318 & 238155 &  5.82 \\
\hline
\end{tabular}
}
\label{table:SS_all}
\end{minipage}
\vspace{-1em}
\end{table}

==> table2.tex <==

\begin{table}[t]
\begin{minipage}{.5\linewidth}
    \centering
    \caption{Privacy impact. \small{R: Real, S: Synthetic}}
    \label{table:PP_all}
    \medskip
\resizebox{1\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c|}{\textbf{DCR}} & \multicolumn{3}{c|}{\textbf{NNDR}} \\
\cline{2-7}
 & \textbf{R\&S} & \textbf{R}  & \textbf{S} & \textbf{R\&S} & \textbf{R}  & \textbf{S}\\

\hline
% \algo 2.0 & 1.056 &  0.428& 0.917 & 0.693 & 0.414 &0.570\\
\algo     & 1.118 &  0.428& 0.937 & 0.713 & 0.414 &0.591\\
CTGAN    & 1.517 &  0.428& 1.026 & 0.763 & 0.414 &0.624 \\
TableGAN & 0.988 &  0.428& 0.920 & 0.681 & 0.414 &0.632\\
MedGAN   & 1.918 &  0.428& 0.254 & 0.871 & 0.414 &0.393 \\
CW-GAN   & 2.197 &  0.428& 1.124 & 0.847 & 0.414 &0.675\\
\hline
\end{tabular}
}
% \label{table:ML_all}
\end{minipage}\hfill
\begin{minipage}{.48\linewidth}
    \centering
    \caption{\small{F1-score difference to CTAB-GAN}}
    % \label{tab:second_table}
    \medskip
    \resizebox{0.9\columnwidth}{!}{
\begin{tabular}{ |C{1.8cm}|C{1.4cm}|C{1.2cm}|C{2.2cm}| C{1.5cm}|}
\hline
\textbf{Dataset} & \textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM and Mode vector}& \textbf{\algo} \\
%\textbf{w/o Classifier} & \textbf{w/o Info. Loss}  & \textbf{w/o VGM} & \textbf{w/o Mode vector} & \textbf{\algo} \\
\hline
 %-0.018&	-0.161& -0.018 &-0.01 & 0.704  \\
% \hline
Adult &  -0.01&	-0.037 & -0.05  & 0.704  \\
\hline
Covertype & -0.018 & -0.184& -0.118  & 0.532\\
\hline
Credit & +0.011& -0.177& +0.06&  0.71 \\
\hline
Intrusion &-0.031&-0.437&+0.003& 0.842 \\
\hline
Loan &-0.044&+0.028&+0.013  & 0.803 \\
\hline
\end{tabular}
}
\label{table:ablation}
\end{minipage}
\vspace{-1em}
\end{table} 

==> table3.tex <==
\begin{table}[t]
\centering
\caption{Training time per epoch.}
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{ |C{2cm}|C{2.4cm}|C{1.8cm}|C{2cm}|C{1.8cm}|C{1.8cm}|C{1.8cm}| }
\hline
\textbf{Dataset} & \textbf{\small{\algo}} &\textbf{\small{\ctgan}} & \textbf{\small{\tablegan}}  & \textbf{\small{\medgan}} & \textbf{\small{\cwgan}}\\ 
\hline
\small{Adult}     & 7.50   &1.66       & 0.52   & 0.33  & 4.73  \\
\hline
 \small Covertype & 8.38    &3.32    & 1.69   & 0.33 & 10.41   \\\hline
\small Credit    & 8.92    &2.42         & 1.73  & 0.34  & 4.50  \\ 
\hline
 \small Intrusion & 10.73    &2.80        & 1.75   & 0.34  & 10.81  \\\hline
\small Loan      & 0.57   &0.17        & 0.06   & 0.04  & 1.12  \\
\hline
\end{tabular}
}
\label{table:training_time}
\vspace{-0.8em}
\end{table}
